Game-Theoretic Analysis of (Non-)Refundable Fees in the Lightning Network

In PCNs, nodes that forward payments between a source and a receiver are paid a small fee if the payment is successful. The fee is a compensation for temporarily committing funds to the payment. However, payments may fail due to insufficient funds or attacks, often after considerable delays of up to several days, leaving a node without compensation. Furthermore, attackers can intentionally cause failed payments, e.g., to infer private information (like channel balances), without any cost in fees. In this paper, we first use extensive form games to formally characterize the conditions that lead to rational intermediaries refusing (or agreeing) to forward payments. A decision made by an intermediary to forward or not depends on the probability of failure, which they approximate based on past experience. We then propose and analyze an alternative fee model that allows the sender to determine and pay a fraction of the fee to intermediaries in a non refundable manner. A rational sender chooses the fraction such that the intermediaries' utility for forwarding the payment exceeds their utility for not forwarding. Our simulation study, based on real world Lightning snapshots, confirms that our novel mechanism can increase the probability of successful payments by 12 percent and decrease routing fees for senders by about 6 percent if all nodes behave rationally. Furthermore, previously cost free probing attacks now require that the attacker pays 1500 satoshis for every 1 million satoshis inferred. Finally, we propose a modification to the Hash Time Locked Contract to enable secure payments of the non refundable fees.

==> Crypto.tex <==

\section{Cryptographic Protocol}\label{seccrypto}
% \csr{figure is in margins, font size is too small}
\begin{figure*}
    \centering
    \input{figures/htlc.tex}
    \caption{Conditional payments in our modified scheme for 4 nodes, one main payment and two for non-refundable fees, tied to the values $r$ chosen by the receiver $v_3$ and $r_0,r_1,r_2$ chosen by the source $v_0$. $\alpha_2=\alpha$ is the payment value, $\alpha_1=\alpha_2+(1-x_2)fee(v_2)$ and $\alpha_0=\alpha_1+(1-x_1)fee(v_1)$. Timelocks excluded for readability.}
    \label{fig:condPay}
\end{figure*}

We have now seen in Section~\ref{results} that having a non-refundable fee increases the success ratio of payments, average fee paid to intermediaies and the cost of conducting a probing attack. Let us now explore how to potentially adjust the cryptographic protocol to accomodate the inclusion of non-refundable fees. The key idea of the adjusted cryptographic protocol is that $v_{i+1}$ provides the preimage that unlocks $v_i$'s non-refundable fee to $v_i$ upon locking the payment value in channel $(v_i, v_{i+1})$. Onion routing is leveraged to provide the preimage, which is chosen by the source, to $v_{i+1}$. We now present an overview of the protocol and argue its security. As our security claims primarily rely on the security of multi-hop payments, aspects such as the choice of timelocks and formal security proofs are analogous~\cite{lightning,kiayias2020composable} and hence excluded from the exposition.


For a path of length $n$, the source initiates $n-1$ HTLC multi-hop payments for non-refundable fees with independent preimages: the $i$th payment is for the $i$th intermediary $v_i$ and is forwarded via the previous intermediaries, conditional on the provision of a preimage of $h(r_i)$ with a random value $r_i$ chosen by the source.

The payment to the receiver contains the payment value and pays the fees (both non-refundable and refundable) to the intermediaries if the payment is successful. This payment is a slight modification of the standard HTLC payment as each conditional payment along the path requires two preimages:  a preimage to $h(r)$ with $r$ chosen by the receiver as in a normal payment and a preimage to $h(r_i)$ with $r_i$ being chosen by the source and provided to $v_i$ by $v_{i+1}$. We call such a payment $HTLC2$. Figure~\ref{fig:condPay} provides an example of all the conditional payments involved. 
The source onion-encrypts the random values $r_0,\ldots ,r_{n-1}$ such that only $v_{i+1}$ can decrypt $r_i$, using the per-hop payload in Lightning's onion routing protocol, which allows the source to send arbitrary information to one specific node~\cite{lightningbolt4}. 

Assume that the main payment is locked in the channel $(v_{i-1}, v_i)$. $v_i$ then decrypts and retrieves $r_{i-1}$, which they forward to their predecessor $v_{i-1}$. They wait until $v_{i-1}$ confirms that $r_{i-1}$ is the correct preimage to their non-refundable fee payment. As a confirmation, $v_{i-1}$ locks the payments for the non-refundable fee payments of $v_{i}, \ldots, v_{n-1}$, i.e., all subsequent intermediaries, in channel $(v_{i-1}, v_i)$.   
Otherwise, the two nodes jointly abort the payment by canceling all corresponding payments in the channel\footnote{we assume that main and fee payments can be linked based on a common id included in the message sent together with the payment}. 
In this manner, the source cannot provide incorrect preimages without the payment being canceled almost immediately. Once the fee payments are locked in channel $(v_{i-1}, v_i)$, $v_i$ initiates a new conditional payment with two values $h(r)$ and $h(r_{i})$ in channel $(v_i,v_{i+1})$, given that the balance of the channel is sufficient to conduct the payment. 
If $v_{i+1}$ is another intermediary, then they in turn provide the preimage $r_i$ to $v_i$ so that $v_i$ can claim its non-refundable fee. After claiming the non-refundable fee, $v_i$ locks the non-refundable fee payments for $v_{i+1}, \ldots, v_{n-1}$ in channel $(v_{i}, v_{i+1})$.  

Once the receiver $v_{n}$ is reached, they provide the preimages $r$ and $r_{n-1}$, the latter being retrieved from the onion-encrypted message. The main payment then completes by forwarding $r$ back to the source, as in a standard HTLC payment. 
Note that the absence of a fee payment to $v_{n}$ reveals that $v_{n}$ is the receiver to $v_{n-1}$. 
To preserve anonymity, the source may set up additional fee payments that can all be claimed by $v_{n}$ through additional preimages included in the message. The total payment value in the main payment can be reduced by the combined value of these fee payments, so that the total amount paid by the source is the same for anonymous and non-anonymous payments. As the receiver should always claim all or none of these payments, atomic multi-path is applied~\cite{osuntokun2018amp}. 

Now, we discuss why the presented protocol allows a node to gain their non-refundable fee even in the presence of misbehaving (but rational) parties. 
As discussed above, the source does not gain anything from providing incorrect preimages. However, an intermediary $v_i$ may be bribed by the source not to provide the preimage to $v_{i-1}$ after the main payment is locked in channel $(v_{i-1}, v_i)$, thus cheating $v_{i-1}$ of its fee. Note that for a rational source, such a bribe is only profitable if it is lower than the non-refundable fee they save when the preimage is not provided. 
We render such an attack unprofitable with the following two conditions: i) Per channel, nodes allow at most one payment for which no preimage for the corresponding non-refundable fee payment is provided. ii) If $v_{i+1}$ does not provide a preimage for the non-refundable fee payment or cancels due to the preimage being incorrect in a timely manner\footnote{what is considered a timely manner is decided by $v_i$, it should take roughly the round trip time to provide the preimage after a payment has been initiated}, its predecessor closes the channel. i) and ii) together guarantee that a node loses at most one non-refundable fee in the whole lifetime of a channel. If a successor is bribed, they lose the channel and opening a new channel is costly, typically more costly than fee for a payment~\cite{lightning} and hence the bribe they gain. So, a rational intermediary does not collude with the source and hence provides the preimage that allows its predecessor to claim the non-refundable fee.

Furthermore, an intermediary $v_i$ should optimally only receive a fee if they lock the payment value in the subsequent channel. However, we can only guarantee this property for an honest successor $v_{i+1}$. Assume that $v_i$ receives its non-refundable fee. Then, $v_i$ has learned the preimage $r_i$, which only the source and $v_{i+1}$ can provide. A rational source does not provide the preimage directly to $v_i$ as this results in the source potentially losing fees. The successor should only provide the preimage if funds are locked, so in case of an honest $v_{i+1}$, $v_i$ indeed only receives funds if they lock. However, if $v_i$ and $v_{i+1}$ collude, $v_{i+1}$ can provide the preimage without locking in exchange for parts of the fee. Requiring a proof of locking does not solve the problem as nodes can always cancel the payment in mutual agreement. This limitation is similar to the wormhole attack in the HTLC protocol that allows colluding intermediaries to claim the fee of other intermediaries~\cite{Malavolta2019AnonymousML}. We accept this limitations for now as --- like the wormhole attack --- it only affects small amounts and only applies in the presence of colluding parties.   





==> ICPADS-Satwik/Background.tex <==
\section{Background}
\label{sec:background}

In this section, we introduce the concepts of payment channel networks and game theory required in our analysis of two routing approaches.   

\subsection{Payment Channel Networks}\label{secpcn}
A payment channel~\cite{decker2015fast} enables two parties to conduct local payments between each other without the need of verifying every payment on-chain while ensuring that both parties can claim the funds that rightfully belong to them. For this, they deposit coins in a shared account. They can then use these coins for local payments. Each payment updates the distribution of coins between the two parties. This distribution is considered private. 
The blockchain acts as a mediator when the two parties disagree on the distribution.

Payment channel networks enable \emph{multi-hop payments} between users that do not share a payment channel network between them without requiring interaction with the blockchain. In such cases, the payment is routed via a path of existing payment channels from a source to a destination~\cite{decker2015fast}.
The Lightning Network (LN)~\cite{lightning} is the payment channel network on top of Bitcoin with more than 15,000 users~\footnotemark[2] .  Multi-hop payments in Lightning are conducted using a source-routed two-phase protocol.   \csp{changed} The receiver generates a payment secret and provides its hash $R$ to the sender. The payment amount is locked in each channel (with information on the hash) from the sender to the receiver. Then, the receiver provides the payment secret to its predecessor. The locked amount in each channel is released in the reverse order from the receiver to the sender once each party receives the payment secret from its successor. In this manner, payments are only finalized once it is known that the payment does reach the receiver. Senders compensate the intermediaries with a small fee if the payment is successful. 

\subsection{Route Finding Protocol}\label{secroute}
In Lightning, all channels are broadcast upon construction and hence the sender has a topology snapshot including the total capacities of all channels as well as the fee and time lock parameters. The sender can use this information to find paths to receivers that have low fees, low timelocks and high probability of success. Dijkstra's algorithm is used to find paths based a custom cost function. The cost function depends on fees, timelocks and success probabilities of the channels in the path. Let $(v_0,v_1,\ldots,v_n)$ be a path with $v_0$ being the source (or payer) and $v_n$ being the destination (or payee) found using \emph{LND}\footnote{\tiny{https://github.com/lightningnetwork/lnd}} (the predominant routing client used by Lightning users) and let $\alpha$ be the amount sent to $v_n$. Let $t_i$ be the timelock of channel $[v_i,v_{i+1}]$ and $\alpha_i$ be the amount being locked in the channel. The fee charged by intermediary $v_i$ is $b_i+\alpha_i\cdot \delta_i$, where $b_i$ is the \emph{base fee} and $\delta_i$ is the \emph{fee rate}. Both values are public and assigned during channel creation. The cheapest path is always constructed from the recipient to the sender. When $v_i$ is being considered to be added to the path, the cheapest sub-path from $v_{i+1}$ to $v_n$ has already been found. Then, the weight of the channel is defined as $weight_i=\alpha_i\cdot t_i\cdot r + f_i $. Here $r$ is a fixed risk factor  and $f_i$ is the fee paid by the sender to $v_i$. Here $\alpha_i\cdot t_i\cdot r$ is referred to as the \emph{timelock penalty}  The sender further makes use of historical knowledge of channel failures to calculate
\begin{equation}\label{eqn:bias}
    bias_i=\frac{Penalty}{\prod_{j=i}^{n-1}p_j}
\end{equation}
where $Penalty$ is set by default to 100 and $p_j$ is the success probability of the channel $[v_j,v_{j+1}]$. The value of $p_j$ is determined based on the time elapsed since the last failure on channel $[v_j,v_{j+1}]$ according to the sender. More precisely,
\begin{equation}\label{eqn:prob}
    p_j = \begin{cases}
                            P_A\cdot(1-\frac{1}{2^{t/t_{1/2}}})& t  \text{ known}\\
                            P_A                      & t \text{ unknown}\\
                    \end{cases}
\end{equation}
where $P_A$ is a channel-independent apriori probability, $t$ is the time elapsed since the last failure in the channel $(v_j,v_{j+1})$ and $t_{1/2}$, also channel independent, determines the rate with which the probability increases over time. The higher the probability, the more likely it is that the sender adds the channel to the payment path. If the payment fails, the sender is able to track at which channel the failure occurred through error messages. 

\subsection{Collateral Cost}\label{seccost}
If a payment fails at $v_{i+1}$, then the payment amount locked by the intermediary $v_i$ may remain locked for the entire duration of the timelock $T_i$.  The opportunity cost of the locked amount during the duration for which the amount is locked is defined as the \emph{collateral cost}~\cite{miller2017sprites} for the intermediary (in units of \emph{time$\times$ money}). Intuitively, the more coins an intermediary locks, the less balance it has available for other payments, meaning it might have to refuse to lock other payments and lose potential routing fees. Similarly, the longer the funds are locked, the more payments might be missed by the intermediary. Thus, the collateral cost for intermediary $v_i$ is $\mathcal{O}(T_i\cdot \alpha_i)$. 

The routing fee acts as a compensation for the collateral cost. Since the collateral cost $c_i$ is $\mathcal{O}(T_i\cdot \alpha_i)$, we can assume that $c_i$ is directly proportional to $T_i\cdot \alpha_i$. This is similar to the timelock penalty we saw in Section~\ref{seccost}. Thus, we quantitatively define the collateral cost similar to the timelock penalty in Section~\ref{secroute} that represents the cost of locking in \emph{LND's} cost function. The only difference would be that intermediaries would use the value of the total timelock from itself to the receiver instead of the timelock of the channel $(v_i,v_{i+1})$ as used in \emph{LND}. The collateral cost $c_i$ for intermediary $v_i$ is thus $T_i\cdot \alpha_i\cdot r$, where $r$ is the \emph{LND} risk factor. 


\subsection{Probing Attacks}\label{secprobing}

Lightning aims to achieve privacy by hiding the balance of a channel from all nodes but the ones adjacent to the channel. In contrast, the capacities of all channels are public information.
Additionally, multi-hop payments in Lightning use onion routing to ensure that any intermediary only knows its predecessor and successor in the path. 


\emph{Probing attacks}~\cite{Biryukov2021probing,probing2019herrera,probing2020gijs,probing2022Nisslmueller,probing2020tikhomorov} aim to infer the balances of specific targeted channels.  
If an intermediary does not lock during the first phase of the payment, it is likely that it lacks the necessary balance to complete the payment. By attempting payments with varying payment amounts, the attacker in a probing attack can infer the balance of the channel. Moreover, the attacker ensures that the payment fails, so that it does not have to pay.  Thus, there is no cost associated with the attack but the collateral cost of locking to the intermediaries. 

The balance $B$ can be estimated using a binary search that iteratively finds a smaller interval $[a,b)$ such that the payments succeeds for $a$, i.e., the balance is sufficient, and fails for $b$, i.e., the balance is insufficient. The initial interval is assumed by the attacker to be $[0,C]$, where $C$ is the total capacity of the target channel. The attack only works under the assumption that intermediaries lock whenever they receive a payment they can handle.  An adversary can use the information on channel balances gained through a probing attack to launch Denial-of-Service attacks like \emph{griefing attacks}~\cite{griefing2020zohar,mizrahi2021congestion,perez2020lockdown,rohrer2019discharged,congestion2020Lu}.

The probing attack in~\cite{probing2022Nisslmueller,probing2019herrera} involves the attacker establishing a channel with a target node whose outgoing balances the attacker wants to determine. An attacker sends invalid payments through the target node to the neighbors of the target node to infer the outgoing balances of the target node with its neighbors. 
% The attacker discovers that the balance of a channel is between $a$ and $b$ when it learns that the channel can route a payment of amount $a$ and not $b$ where $b>a$.
This attack is improved by utilizing both directions of a channel to probe balances~\cite{probing2020gijs}. Sending  payments over longer paths can be used to probe balances of multiple channels along the path by determining which channel was responsible for the failure~\cite{probing2020tikhomorov}. Finally, recent work in~\cite{Biryukov2021probing} also accounts for multiple channels between two nodes while probing.


% %Additionally, the anonymity of senders and recipients are protected by using onion routing and hence intermediaries are only aware of its immediate neighbors in the path. 
% A more detailed description on the working of payment channels and payment channel networks is provided in Appendix~\ref{appPCN}. 

\subsection{Detailed Game-Theoretical Background}\label{secgame}


%As multiple concepts are illustrated in the figure, not all of them are defined when Figure~\ref{fig4} is first mentioned in the text. 

A game here is a situation whose outcome depends on the actions of multiple parties (called players). All players aim to optimize their \emph{utility}, i.e., they assign each outcome a value of how beneficial the outcome is for them and aim to maximize this value. The outcome of the game is then represented as a vector of utilities, one for each player. Note that we use the terms players and parties interchangeably and both mean the same thing. We use Figure~\ref{fig4} to illustrate the concepts introduced in this section. \csg{this seems enough to me}

The outcome of a multi-hop payment depends on the actions of the payer, payee, and intermediaries. Decisions are made sequentially in multi-hop payments, i.e., locking and payment decisions are made one after the other. We can hence use \emph{extensive form games}, which model games as a sequence of decisions, with each sequence of decisions having a particular outcome. Typically, an extensive form game is represented as a \emph{game tree}. The internal nodes of the tree correspond to decisions and are labelled by the name of the player who makes the decision. For instance, in Figure~\ref{fig4}, the root node corresponds to a decision made by $A$ between options $G$ and $H$. $G$ leads to an outcome while $H$ is followed by decisions of other players. 
A link represents an option for a decision leading to a new decision or a final outcome. The link is labelled by the option. Final outcomes, resulting from a sequence of decisions, are represented by leaf nodes. The utilities for every player corresponding to an outcome are represented as a tuple at the corresponding leaf node.


\begin{figure}
	% \vspace{-2em}
	\centering
	\begin{istgame}[font = \tiny,scale = 0.4] %\setistgrowdirection'{east} 
		\xtdistance{15mm}{30mm} 
		\istroot(0){A}
		\istb{G}[al]{(0,2)}
		\istb{H}[ar]
		\endist
		\istroot(1)(0-2)<above right>{N}
		\istb{S1}[al]
		\istb{S2}[ar]
		\endist
		\xtdistance{15mm}{30mm}
		\istroot(2)(1-1)
		\istb{I}[al]{(2,2)}
		\istb{J}[ar]{(-2,-2)}
		\endist
		\istroot(3)(1-2)
		\istb{I}[al]{(-2,-2)}
		\istb{J}[ar]{(2,2)}
		\endist
		\xtInfoset(2)(3){B}
	\end{istgame}
	\vspace{-0.5em}
	\caption{Illustration of basic game-theoretical concepts }
	%	Game between players $A$ and $B$. $A$ has options $G$, which leads to utility $(0,2)$, and $H$. If $A$ chooses $H$, then $B$ has to decide between $I$ and $J$. The utilities for $B$ (and $A$) are not fully known if $A$ chooses $H$, they can be either $(2,2)$ for $I$ (Scenario $S1$) and $(-2,-2)$ for $J$ or vice versa (Scenario $S2$). We can turn this game from a game with incomplete information into one with imperfect information  assuming that an external entity or \emph{Nature} ($N$) decides whether we are in $S1$ or $S2$.
	
	\label{fig4}
	\vspace{-2.5em}
\end{figure}

%For instance, in a direct payment between a payer $p_1$ and a payee $p_2$, the root node of the tree is the decision of $p_1$ to pay or not. If $p_1$ decides not to pay, the game ends and both parties' utility is zero. Thus, in the game tree, there is an edge from the root node to the outcome $(0,0)$. A second edge represents $p_1$'s decision to pay and leads to a node representing $p_2$'s decision to accept the payment. Two edges lead to two final outcomes, one corresponding to $p_2$ accepting and one for $p_2$ declining. 

Extensive form games differ based on the amount of information the players have. 
The first aspect to consider is whether a player making a decision is aware of all previous decisions. If that is the case for all players, the game has \emph{perfect information}, otherwise it has \emph{imperfect information}. In the game tree, we connect nodes of the same player with a dotted line if the player cannot tell at which node of the game tree the player is making the decision. 

A game has \emph{complete information} if all players know the exact utilities of each outcome and the \emph{type} (e.g., rational, byzantine) of the other players.
Otherwise, the game has \emph{incomplete information}. In a game with incomplete information, there are essentially multiple game trees, one for each possible set of utilities and types. The game can be turned from a game with incomplete information into a game with imperfect information as illustrated in Figure~\ref{fig4}. 
When a decision made by player $P$ has multiple possible outcomes, we add a node with the player called \emph{Nature} to the game tree. Nature represents an external entity that makes random decisions between different scenarios. For each possible outcome, we then add a child labelled $P$ to the Nature's decision.
While the children have the same options available, the options lead to different outcomes. $P$ is unaware which decision \emph{Nature} made and hence does not know in which scenario it is, as in a game with imperfect information.
Figure~\ref{fig4} provides an example. Here, the utilities for $B$ (and $A$) are not fully known if $A$ chooses $H$, they can be either $(2,2)$ for $I$ and $(-2,-2)$ for $J$ if $N$ chooses $S1$ or vice versa if $N$ chooses $S2$ . An external entity \emph{Nature} ($N$) decides whether we are in $S1$ or $S2$.







We now turn to how players make decisions in a game. 
The decisions made by a player throughout the game are the player's \emph{strategy}. One decision is a \emph{move}. A \emph{dominant} strategy is one that achieves a better utility than other alternative strategies, regardless of the actions of the other players.  
A \emph{strategy profile} is the set of strategies used by all the players in the game. 
A \emph{Nash equilibrium} is a strategy profile such that no single player can improve their utility by deviating from their strategy. 

For an extensive form game with perfect and complete information, we can find a Nash equilibrium through \emph{backward induction}. Backward induction starts from the player who represents the leaf node or the last player who chooses the strategy that is most beneficial to itself. The second-to-last player can then predict the last player's strategy (since the game is perfect and has complete information) and can choose its best strategy. In this manner, each player predicts the best strategies of the subsequent players and chooses its best strategy.
% In each round, backward propagation considers a node such that all the nodes’ children have an outcome
% assigned. Let $P$ be the player associated with the node.  
% Of all of the moves available to $P$, we then assign the one that is most beneficial to $P$ to the node. Initially, only the leaf nodes can, with the other nodes receiving their outcomes iteratively after their children have been assigned outcomes. 
The strategy profile corresponding to the one given by decisions chosen during backward induction forms a Nash equilibrium. 

For a game with imperfect information (and hence also for a game with incomplete information), we can use a variant of backward induction that considers expected utilities instead of exact utilities. In order to be able to compute expected utilities, nodes need to have a \emph{belief} about the decisions previously made. Concretely, when uncertain about which node they are at, a player $P$ assigns each potential node a probability, computes the utilities for all of them, and then computes the expected value of these utilities. $P$ chooses the decision with the highest expected utility. 
We can then say that $P$ is acting in a \emph{sequentially rational} manner, \emph{consistent} with their beliefs. The result of all players applying this method is a \emph{Bayesian Nash equilibrium}. 

For instance, in Figure~\ref{fig4}, assume node $B$ assigns probability $q$ to $S1$ and $1-q$ to $S2$ as its belief of $N$'s choice. Then the expected utility for $B$ on choosing $I$ is $2\cdot q -2\cdot (1-q) = 4\cdot q-2$ and similarly the expected utility on choosing $J$ is $2-4\cdot q$. So $B$ chooses $I$ if $q>0.5$ and $J$ if $q<0.5$. 

$A$ in turn has its own belief about what $N$ will choose and also about what $B$ believes (about $q$). Let $q_1$ and $1-q_1$ be the probabilities that $A$ assigns to $S1$ and $S_2$, respectively. Also, let $q_2$ and $1-q_2$ be the probabilities that $A$ assigns to whether $B$ believes $q>0.5$ or $q<0.5$ respectively. After $N$ chooses $S1$, $A$'s expected utility is calculated to be $4\cdot q_2 - 2$.  Similarly, after $N$ chooses $S2$,  $A$'s expected utility is $2-4\cdot q_2$. Thus, $A$'s overall expected utility $u$ on choosing $H$, based on its beliefs, is $q_1\cdot (4\cdot q_2 - 2) + (1-q_1)\cdot(2-4\cdot q_2)$. Since, $A$'s utility on choosing $G$ is $0$, it chooses $H$ only if $u>0$. \csg{I can't find what $u$ means}

Thus far, we have only dealt with \emph{pure} strategies, i.e., each player chooses an action for sure. A player may employ a \emph{mixed} strategy, where it assigns a probability distribution over its set of pure strategies and selects its strategy based on the distribution. For example, in Figure~\ref{fig4}, this means that $A$ chooses $G$ and $H$ with probabilities $p_G$ and $p_H$, respectively ($p_G + p_H=1$).  $A$ assigns $p_G$ (and $p_H$) such that its expected utility $p_G\cdot U_G +p_H\cdot U_H$ is maximized given the values of $q_1$ and $q_2$. Here, $U_G$ and $U_H$ are utilities $A$ obtains by choosing $G$ and $H$, respectively. Similarly, $B$ also assigns a probability distribution over $I$ and $J$ depending on $q$. When each player maximizes their respective utilities, a Bayesian Nash equilibrium is reached.



  % Throughout the paper, we mainly\csr{why mainly?} consider processes that involve multiple parties making strategic decisions. We now introduce game-theoretic concepts that we need to study the optimal behavior of parties. In order to capture parties making strategic decisions sequentially we use the graphical representation of games, which is called a \emph{game tree}. An \emph{extensive form game} is used to explicitly represent the key aspects of a game like sequence of moves, choices at each decision point, the information available to each party when making a move and the payoffs for each party at every outcome. \csr{don't you need requirements on games to do so?}

% \begin{figure}
% \centering
% \begin{istgame}
% \xtdistance{15mm}{30mm}
%   \istroot(0){$A$}
%      \istb{$G$}[above left]{(0,2)}
%      \istb{$H$}[above right]
%      \endist
%   \istroot(1)(0-2)<30>{$B$}
%      \istb{$I$}[al]{(1,1)}
%      \istb{$J$}[ar]{(-1,-1)}
%      \endist
%   \end{istgame}
%   \caption{Example of an extensive form game with two players $A$ and $B$. $A$ first makes a move by choosing between $G$ and $H$. $B$ then follows up by choosing between $I$ and $J$. Each leaf node represents the utilities for each player for each sequence of moves. For example, if $A$ chooses $H$ and $B$ chooses $F$, then both $A$ and $B$ get a utility of $1$.}
%   \label{fig1}
%   \end{figure}

% Figure~\ref{fig1} shows an example of an extensive form game. The above example is a game with both \emph{perfect information} and \emph{complete information}. By perfect information, we mean that at any stage of the game, each player knows the exact sequence of prior moves. By complete information, we mean that each each player knows the exact utilities at each outcome and the \emph{type} (rational, byzantine etc.) of the other players. 

% \emph{Nash equilibrium} is a common way to describe the expected behavior of a game involving two or more players. A strategy profile is a set of strategies, one for each player. Intuitively, a Nash equilibrium is a strategy profile such that no party gains anything by unilaterally deviating from its strategy. 

% If we consider the game in Figure~\ref{fig1}, we can see that player $B$'s utility when choosing $I$ rather than $J$, regardless of $A$'s choice. $J$ is then a \emph{dominated strategy}. $A$ can expect this behavior from $B$ and we can see that $A$'s utility is higher when choosing $H$ rather than $G$, making $G$ a dominated strategy. Thus, when $A$ chooses $H$ and $B$ chooses $I$, both players cannot make gains by unilaterally deviating from this strategy and thus the strategy profile $\{H,I\}$ is a Nash equilibrium. This method of finding the Nash equilibrium by eliminating dominated strategies as we iterate from the last player to the first player making a move is called \emph{backward induction}. Backward induction cannot be used for games with \emph{imperfect} or \emph{incomplete} information. 

% \begin{figure}
%     \centering

% \begin{istgame} %\setistgrowdirection'{east} 
% \xtdistance{15mm}{30mm} \istroot(0){A}
%   \istb{A}[al]{(2,2)}
%   \istb{D}[ar]
%   \endist
% \istroot(1)(0-2)<above right>{A}
%   \istb{L}[al]
%   \istb{R}[ar]
%   \endist
% \xtdistance{10mm}{20mm}
% \istroot(2)(1-1)
%   \istb{\ell}[al]{(4,2)}
%   \istb{r}[ar]{(1,1)}
%   \endist
% \istroot(3)(1-2)
%   \istb{\ell}[al]{(3,2)}
%   \istb{r}[ar]{(2,3)}
%   \endist
% \xtInfoset(2)(3){B}
% \end{istgame}
% \caption{Example of a game with imperfect information. Here player $B$ does not know whether in the previous move, $A$ played $L$ or $R$. The dotted line represents an \emph{information set} with two nodes. $B$ cannot tell at which node of the information set it is at.}
% \label{fig2}
% \end{figure}

% The game in Figure~\ref{fig2} is an example of imperfect information. In this case, $B$ needs to have a \emph{belief} on the probability of being at any particular node of an information set to strategize its best move. In this case, let $B$'s belief be that $A$ plays $L$ with probability $p$ and $R$ with probability $1-p$, then $B$'s expected utility on playing $l$ is $p\cdot 2 + (1-p)\cdot 1 = p+1$ and on playing $r$ is $p\cdot 1 +(1-p)\cdot 3 = 3-2\cdot p$. Based on the value of $p$ that is assumed by $B$, it chooses the strategy that maximizes its expected utility. Here, $B$ is acting in a \emph{sequentially rational} manner, \emph{consistent} with its beliefs. Similarly, let $A$'s belief be that $B$ plays $l$ with probability $q$ and $r$ with probability $1-q$. Then, $A$'s expected utility on playing $L$ is $q\cdot 4 + (1-q)\cdot 1 = 4\cdot q+1$ and on playing $R$ is $q\cdot 3+(1-q)\cdot 2 = q+3$. Since $q>0$, we have $4\cdot q+1>3q$ and $A$ always prefers to play $L$. Based on the value of $q$ assumed by $A$, it chooses the strategy that maximizes its expected utility. Let us suppose, $4\cdot q+1>q+3$ and thus, $A$ prefers $L$ over $R$ in the second step, then in the first step, $A$ chooses $D$ if $4\cdot q+1 > 2$. 

% \begin{figure}
%     \centering
%     \subfloat[Scenario 1]{
%     \begin{istgame}
% \xtdistance{10mm}{20mm}
%   \istroot(0){$A$}
%      \istb{$G$}[above left]{(0,2)}
%      \istb{$H$}[above right]
%      \endist
%   \istroot(1)(0-2)<30>{$B$}
%      \istb{$I$}[al]{(2,2)}
%      \istb{$J$}[ar]{(-2,-2)}
%      \endist
%   \end{istgame}}
%   \subfloat[Scenario 2]{
%     \begin{istgame}
% \xtdistance{10mm}{20mm}
%   \istroot(0){$A$}
%      \istb{$G$}[above left]{(0,2)}
%      \istb{$H$}[above right]
%      \endist
%   \istroot(1)(0-2)<30>{$B$}
%      \istb{$I$}[al]{(-2,-2)}
%      \istb{$J$}[ar]{(2,2)}
%      \endist
%   \end{istgame}}
%     \caption{Example of an incomplete information game. Here $B$ does not know whether it is in Scenario 1 or Scenario 2 and hence cannot directly estimate its utility on choosing $I$ or $J$}.
%     \label{fig3}
% \end{figure}
 
% Figure~\ref{fig3} shows an example of an incomplete information game. Such incomplete information games can be represented using an imperfect information extensive form game using the Harsanyi transformation as seen in Figure~\ref{fig4}. 



% If all parties act to maximize their expected utilities given their beliefs and other parties equilibrium strategies, we have a \emph{Bayesian Nash equilibrium}. 

==> ICPADS-Satwik/Conclusion.tex <==
\section{Conclusion}

Lightning's current incentive model falls short of providing incentives to intermediaries when payments fail. We proposed a modified incentives model in which intermediaries are guaranteed partial fees (payed by the sender) for locking payments and analyze both models formally using extensive form games. In the future, we will consider incentives for alternative models of multi-hop payments in payment networks including constant and linear collateral payments~\cite{miller2017sprites,Egger2019amcu,jourenko2021trees}, single-phase payments~\cite{blitz}, and local routing~\cite{speedymurmurs,silentwhispers,robustpay} as well as the design of cryptographic algorithms enforcing advance fees. 

  




==> ICPADS-Satwik/Crypto.tex <==

\section{Cryptographic Protocol}\label{seccrypto}
% \csr{figure is in margins, font size is too small}
\begin{figure*}
    \centering
    \input{figures/htlc.tex}
    \caption{Conditional payments in our modified scheme for 4 nodes, one main payment and two for non-refundable fees, tied to the values $r$ chosen by the receiver $v_3$ and $r_0,r_1,r_2$ chosen by the source $v_0$. $\alpha_2=\alpha$ is the payment value, $\alpha_1=\alpha_2+(1-x_2)fee(v_2)$ and $\alpha_0=\alpha_1+(1-x_1)fee(v_1)$. Timelocks excluded for readability.}
    \label{fig:condPay}
\end{figure*}

We have now seen in Section~\ref{results} that having a non-refundable fee increases the success ratio of payments, average fee paid to intermediaies and the cost of conducting a probing attack. Let us now explore how to potentially adjust the cryptographic protocol to accomodate the inclusion of non-refundable fees. The key idea of the adjusted cryptographic protocol is that $v_{i+1}$ provides the preimage that unlocks $v_i$'s non-refundable fee to $v_i$ upon locking the payment value in channel $(v_i, v_{i+1})$. Onion routing is leveraged to provide the preimage, which is chosen by the source, to $v_{i+1}$. We now present an overview of the protocol and argue its security. As our security claims primarily rely on the security of multi-hop payments, aspects such as the choice of timelocks and formal security proofs are analogous~\cite{lightning,kiayias2020composable} and hence excluded from the exposition.


For a path of length $n$, the source initiates $n-1$ HTLC multi-hop payments for non-refundable fees with independent preimages: the $i$th payment is for the $i$th intermediary $v_i$ and is forwarded via the previous intermediaries, conditional on the provision of a preimage of $h(r_i)$ with a random value $r_i$ chosen by the source.

The payment to the receiver contains the payment value and pays the fees (both non-refundable and refundable) to the intermediaries if the payment is successful. This payment is a slight modification of the standard HTLC payment as each conditional payment along the path requires two preimages:  a preimage to $h(r)$ with $r$ chosen by the receiver as in a normal payment and a preimage to $h(r_i)$ with $r_i$ being chosen by the source and provided to $v_i$ by $v_{i+1}$. We call such a payment $HTLC2$. Figure~\ref{fig:condPay} provides an example of all the conditional payments involved. 
The source onion-encrypts the random values $r_0,\ldots ,r_{n-1}$ such that only $v_{i+1}$ can decrypt $r_i$, using the per-hop payload in Lightning's onion routing protocol, which allows the source to send arbitrary information to one specific node~\cite{lightningbolt4}. 

Assume that the main payment is locked in the channel $(v_{i-1}, v_i)$. $v_i$ then decrypts and retrieves $r_{i-1}$, which they forward to their predecessor $v_{i-1}$. They wait until $v_{i-1}$ confirms that $r_{i-1}$ is the correct preimage to their non-refundable fee payment. As a confirmation, $v_{i-1}$ locks the payments for the non-refundable fee payments of $v_{i}, \ldots, v_{n-1}$, i.e., all subsequent intermediaries, in channel $(v_{i-1}, v_i)$.   
Otherwise, the two nodes jointly abort the payment by canceling all corresponding payments in the channel\footnote{we assume that main and fee payments can be linked based on a common id included in the message sent together with the payment}. 
In this manner, the source cannot provide incorrect preimages without the payment being canceled almost immediately. Once the fee payments are locked in channel $(v_{i-1}, v_i)$, $v_i$ initiates a new conditional payment with two values $h(r)$ and $h(r_{i})$ in channel $(v_i,v_{i+1})$, given that the balance of the channel is sufficient to conduct the payment. 
If $v_{i+1}$ is another intermediary, then they in turn provide the preimage $r_i$ to $v_i$ so that $v_i$ can claim its non-refundable fee. After claiming the non-refundable fee, $v_i$ locks the non-refundable fee payments for $v_{i+1}, \ldots, v_{n-1}$ in channel $(v_{i}, v_{i+1})$.  

Once the receiver $v_{n}$ is reached, they provide the preimages $r$ and $r_{n-1}$, the latter being retrieved from the onion-encrypted message. The main payment then completes by forwarding $r$ back to the source, as in a standard HTLC payment. 
Note that the absence of a fee payment to $v_{n}$ reveals that $v_{n}$ is the receiver to $v_{n-1}$. 
To preserve anonymity, the source may set up additional fee payments that can all be claimed by $v_{n}$ through additional preimages included in the message. The total payment value in the main payment can be reduced by the combined value of these fee payments, so that the total amount paid by the source is the same for anonymous and non-anonymous payments. As the receiver should always claim all or none of these payments, atomic multi-path is applied~\cite{osuntokun2018amp}. 

Now, we discuss why the presented protocol allows a node to gain their non-refundable fee even in the presence of misbehaving (but rational) parties. 
As discussed above, the source does not gain anything from providing incorrect preimages. However, an intermediary $v_i$ may be bribed by the source not to provide the preimage to $v_{i-1}$ after the main payment is locked in channel $(v_{i-1}, v_i)$, thus cheating $v_{i-1}$ of its fee. Note that for a rational source, such a bribe is only profitable if it is lower than the non-refundable fee they save when the preimage is not provided. 
We render such an attack unprofitable with the following two conditions: i) Per channel, nodes allow at most one payment for which no preimage for the corresponding non-refundable fee payment is provided. ii) If $v_{i+1}$ does not provide a preimage for the non-refundable fee payment or cancels due to the preimage being incorrect in a timely manner\footnote{what is considered a timely manner is decided by $v_i$, it should take roughly the round trip time to provide the preimage after a payment has been initiated}, its predecessor closes the channel. i) and ii) together guarantee that a node loses at most one non-refundable fee in the whole lifetime of a channel. If a successor is bribed, they lose the channel and opening a new channel is costly, typically more costly than fee for a payment~\cite{lightning} and hence the bribe they gain. So, a rational intermediary does not collude with the source and hence provides the preimage that allows its predecessor to claim the non-refundable fee.

Furthermore, an intermediary $v_i$ should optimally only receive a fee if they lock the payment value in the subsequent channel. However, we can only guarantee this property for an honest successor $v_{i+1}$. Assume that $v_i$ receives its non-refundable fee. Then, $v_i$ has learned the preimage $r_i$, which only the source and $v_{i+1}$ can provide. A rational source does not provide the preimage directly to $v_i$ as this results in the source potentially losing fees. The successor should only provide the preimage if funds are locked, so in case of an honest $v_{i+1}$, $v_i$ indeed only receives funds if they lock. However, if $v_i$ and $v_{i+1}$ collude, $v_{i+1}$ can provide the preimage without locking in exchange for parts of the fee. Requiring a proof of locking does not solve the problem as nodes can always cancel the payment in mutual agreement. This limitation is similar to the wormhole attack in the HTLC protocol that allows colluding intermediaries to claim the fee of other intermediaries~\cite{Malavolta2019AnonymousML}. We accept this limitations for now as --- like the wormhole attack --- it only affects small amounts and only applies in the presence of colluding parties.   





==> ICPADS-Satwik/Evaluation.tex <==
\section{Evaluation}
\label{sec:evaluation}

In this section, we evaluate Lightning's and the modified incentive model in terms of the success ratio of multi-hop payments, the additional income to the intermediaries as well as the increase in cost for the senders. We also experimentally determine the amount of fees that a malicious sender has to pay when conducting a probing attack in our new incentive model. 
% \begin{figure*}
%     \centering
%     \subfloat[\emph{\textbf{$SR$ for $Pr_A = 0.8$}}]{\includegraphics[scale=0.20]{Tex/figures/SR8.png}\label{SR8}} \hfill 
%     \subfloat[\emph{\textbf{$LR$ for $Pr_A = 0.8$}}]{\includegraphics[scale=0.20]{Tex/figures/LR8.png}\label{LR8}}\hfill
%     \subfloat[\emph{\textbf{$Fee_I/C$ for $Pr_A = 0.8$}}]{\includegraphics[scale=0.20]{Tex/figures/FI8.png}\label{FI8}}\hfill
%     \subfloat[\emph{\textbf{$Fee_S$ for $Pr_A = 0.8$}}]{\includegraphics[scale=0.20]{Tex/figures/FS8.png}\label{FS8}}\hfill
%     \subfloat[\emph{\textbf{$SR$ for $Pr_A = 0.9$}}]{\includegraphics[scale=0.20]{Tex/figures/SR9.png}\label{SR9}}\hfill
%     \subfloat[\emph{\textbf{$LR$ for $Pr_A = 0.9$}}]{\includegraphics[scale=0.20]{Tex/figures/LR9.png}\label{LR9}}\hfill
%     \subfloat[\emph{\textbf{$Fee_I/C$ for $Pr_A = 0.9$}}]{\includegraphics[scale=0.20]{Tex/figures/FI9.png}\label{FI9}}\hfill
%     \subfloat[\emph{\textbf{$Fee_S$ for $Pr_A = 0.9$}}]{\includegraphics[scale=0.20]{Tex/figures/FS9.png}\label{FS9}}\hfill
%     \caption{Comparison of $SR$,$LR$,$Fee_I/C$ and $Fee_S$ values for different selections of $\tau$,$Pr_A$ and $r$ for original and modified protocols}
%     \label{fig:1}
% \end{figure*}
\subsection{Simulation setup}\label{simmodel}
Note that we did not specify how to exactly calculate the perceived probabilities of payment success ($p^i_S$,$p'^i_S$ and $P^i_S$ from Sections~\ref{rout},~\ref{sec:modifiedgame}). They are based on past observation but there are multiple ways to weight observations, e.g., based on how in the past they occurred. 
We choose a simple solution for our experiments that is in line with Lightning's general treatment of failures.  
Afterwards, we provide details about how transactions are executed in our setup. 

% \textbf{Path selection:}
% In Lightning, all channels are broadcast upon construction and hence the sender has a topology snapshot including the total capacities of all channels as well as the fee and timelock parameters. Based on the snapshot, we select a path between the sender and the recipient. We use the path selection algorithm from LND, the most popular Lightning client, to find a path from the sender to the recipient of a payment. The main idea of the algorithm is that the sender determines the best path using Dijkstra's algorithm based on a cost function (depending on fees, timelocks and success probabilities of each hop).

% One aspect of LND's cost function, which we are extending for our success probabilities, is that it includes the time since the last failure. Each channel is assigned a success probability based on its past failures:
% \begin{equation}\label{eq:p}
%         P[v_i,v_{i+1}] = \begin{cases}
%                             P_A\cdot(1-\frac{1}{2^{t/t_{1/2}}})& t  \text{ known}\\
%                             P_A                      & t \text{ unknown}\\
%                     \end{cases}
%     \end{equation}
%     where $P_A$ is a channel-independent apriori probability, $t$ is the time elapsed since the last failure in the channel $(v_i,v_{i+1})$ and $t_{1/2}$, also channel independent, determines the rate with which the probability increases over time. The higher the probability, the more likely it is that the sender adds the channel to the payment path. If the payment fails, the sender is able to track at which channel the failure occurred. The point in time of the last failure is updated with every failure.

\textbf{Calculation of success probabilities:}
The probabilities $p^i_S$, $P^i_S$ and $\Tilde{p}^i_S$ are calculated in a similar manner as in Eq.~\ref{eqn:prob}. We only consider the last failure instead of, e.g., the frequency of failures, because only the last failure is indicative of the current available funds.
%$p^i_S$, $P^i_S$ and $p'^i_S$ 
These three probabilities use different values of $t$ and $t_{1/2}$ in Eq.~\ref{eqn:prob}:
an intermediary $v_i$ calculates $p^i_S$ with the value of $t$ being the time since the last payment failed after $v_i$ forwarded a payment to $v_{i+1}$, 
the sender $v_0$ calculates $\Tilde{p}^i_S$ with the value of $t$ being the time 
since the last failure of a payment sent by $v_0$ after $v_i$ locked with $v_{i+1}$, and finally, the sender $v_0$ calculates $P_S^i$ with $t$ being the time since the last failure of a payment sent by $v_0$ caused by $v_i$ refusing to lock with $v_{i+1}$. The sender uses $P_S^i$ to calculate the value of the buffer $d_i$ for $v_i$ with $d_i=0.1\cdot (1-P_S^i)$ so that $d_i$ decrease after $v_i$ locks and increases when $v_i$ does not lock.

We use two different constant values of $t_{1/2}$, one for the intermediaries denoted by $t_{1/2}^I$, and one for senders denoted by $t_{1/2}^S$.  
The value of $t_{1/2}^S$ is always chosen to be higher than $t_{1/2}^I$ to make up for the fact that the sender is unaware of some failures. Hence, it needs to consider the failures it is aware of 
with a higher weight. 
The value of $P_A$ is identical for senders and intermediaries.

\textbf{Payment execution:}
We build on the Python package \emph{Networkx} to simulate a payment channel network and multi-hop payments in the network. 
We did not simulate the cryptographic protocols in order to increase scalability. 
Payments are executed sequentially and assumed to complete --- successfully or not --- immediately.
Having concurrency merely might reduce the success ratio as payments may block each other, but the effect has been shown to be small in comparison to changing the average payment value~\cite{eckey2020splitting}. 
In order to still have a notion of time required for computing the success probabilities, we assume there is a uniformly random delay between two consecutive payments. 


% All players make decisions based on the expected utilities of the routing games discussed in Section~\ref{rout} and~\ref{sec:modifiedgame}. 

Once the sender finds a path based on LND's path finding algorithm, all players make decisions based on their respective expected utilities in the routing games discussed in Section~\ref{rout} and~\ref{sec:modifiedgame}. When a payment fails, the intermediaries who chose $L$ and the sender record this failure and use this knowledge to compute the success probabilities for future payments. If modified incentives are used, then the sender pays partial fees to the intermediaries who have chosen $L$.  
% In the beginning of each payment, the sender finds a path using LND's path finding algorithm and locks the payment value (including the fees of all intermediaries) in its channel with the first intermediary. Then, every intermediary chooses $L$ or $NL$ (depending on its expected utility and availability of balance). If all intermediaries of a payment choose $L$, the payment succeeds and the balances are changed accordingly. A payment fails if an intermediary chooses $NL$ (either due to insufficient balance or if it deems its expected utility on participation to be negative \csg{why change the order of the reasons?}). When a payment fails, the intermediaries who chose $L$ and the sender record this failure and use this knowledge to compute the success probabilities for future payments. If modified incentives are used, then the sender pays partial fees to the intermediaries who have chosen $L$. 
%We simulate concurrent payments by executing payments in rounds (the number of rounds elapsed is a measure of the time elapsed). A random number of payments are attempted in every round. If all intermediaries of a payment choose $L$, the payment succeeds in the same round as it was attempted and the balances of the channels involved are changed accordingly. If any intermediary chooses $NL$ due to insufficient balance (the intermediary expects a positive utility), the payment is kept on hold\csr{I don't think this is how Lightning works???} until either 1) the intermediary's balance is replenished, by other payment(s), and the payment is forwarded to its successor or 2) the timelocks, of parties who chose $L$, expires and the payment fails. Otherwise, the payment fails after the timelocks expire.\csr{unclear to me what otherwise is for}
%
%\csr{I don't fully understand that round thing...how do you deal with payments that take varying numbers of hops?}
%When a payment fails, intermediaries note the round in which they confirmed the failed payment as the last instance to failure. The sender is also informed of the point of failure so that it can pay the non-refundable portion of the fees to the intermediaries who chose $L$. Knowing the point of failure, the sender also estimates the instances at which every intermediary who chose $L$ noted the failure and uses this knowledge to estimate the non-refundable fees for future payments.

To capture the event where the sender of a payment uses knowledge of past channel failures to adjust the values of $x_i$ for every intermediary, we need multiple payment attempts from the same sender over the same intermediary at different points of time. In our simulations, we obtain such repeated scenarios at a faster rate when we impose a restriction on the set of possible senders and recipients. Hence, we sample a small subset $\omega$ of all the nodes in the network and the sender-recipient pair for every payment are sampled from $\omega$ to save simulation time and yet capture the essential working of the routing game. \csp{New} Meaningful results can be obtained for bigger subsets by simulating a lot more payments. We expect the results to be similar as parties update their strategies only based on the payments they observe.%We do not bias the results of our evaluation in doing so because we can think of payments between senders/recipients from a smaller subset of nodes as a subset of all payments in the network.Consequently, we evaluate the success ratio of payments, rate of intermediaries choosing $L$ and the gains/losses of intermediaries limited to the above-mentioned subset of payments. The evaluation can be extended to include payments between all sender/recipient pairs given more simulation time.  \csr{can you argue that this does not bias the results?}\csp{I tried to argue now}

\subsection{Metrics}\label{metrics}
We use the following metrics to evaluate both the original and modified incentives: 1) The ratio of the number of payments that succeed to the number of payments attempted is the \emph{success ratio} $SR$, 2) The ratio of the number of moves by intermediaries that are $L$ to the number of all the moves made by intermediaries is the \emph{lock ratio} $LR$, 3) The average fee collected by the intermediaries, over all payments that they participate in whether by locking or not locking is called $F_I$ (in satoshis), 4) The average fee paid by the senders,  over all payments they started, is called $F_S$ (in satoshis), 5) The average non-refundable fee gained per intermediary over all failed payments is called $F'_I$(in satoshis), 6) The average non-refundable fee gained per intermediary over all failed payments is called $F'_S$(in satoshis).
% \csg{why do the first two metrics have names and the latter two do not? Check last two definitions}\csp{updated}
% \begin{itemize}
%     \item The ratio of the number of payments that succeed to the number of payments attempted is the \emph{success ratio} $SR$.
%     \item The ratio of the number of moves by intermediaries that are $L$ to the number of all the moves made by intermediaries is the \emph{lock ratio} $LR$. 
%     \item The average fee collected by intermediaries, \csg{not: the intermediaries?} over all payments that they participate \csg{not: they participate?} in whether by locking or not locking is called $F_I$ (in satoshis).
%     \item The average fee paid by the senders, \csg{not: the senders?} over all payments they started, \csg{they started} is called $F_S$ (in satoshis).
% \end{itemize}



\subsection{Parameters}\label{secparameters}

\begin{table*}
	\begin {center}
	\begin{tabular}{c r@{$\pm$}l r@{$\pm$}l r@{$\pm$}l r@{$\pm$}l r@{$\pm$}l r@{$\pm$}l}
		\toprule
		\textit{Cases} 
		& \multicolumn{2}{c}{$SR$} 
		& \multicolumn{2}{c}{$LR$}
		& \multicolumn{2}{c}{$F_I$}
		& \multicolumn{2}{c}{$F_S$}
		& \multicolumn{2}{c}{$F'_I$}
		& \multicolumn{2}{c}{$F'_S$}\\
		\midrule
		\textbf{\textit{Original}} & 0.65&0.11 & 0.70&0.11 & 2.92&0.22&11.26&1.86&0&0&0&0\\
		\textbf{\textit{ModGuaranteed}} & 0.73&0.08 & 0.81&0.07 & 2.67&0.22&10.52&1.85&1.37&0.3&2.63&0.52\\
		\textbf{\textit{ModIncentivized}} & 0.71&0.09 & 0.78&0.08 &2.65&0.27 &10.64&1.94&0.37&0.12&0.73&0.27\\
		\bottomrule
	\end{tabular}
 \vspace{-0.5em}
	\caption{Comparison of metrics in the three cases Original, ModGuaranteed, and ModIncentivized. Each entry comprises of the mean and the standard deviation of the metric averaged across the 10 sets of payments for the corresponding case.}
    \label{table}
	\end {center}
 \vspace{-3em}
\end{table*}
% \csr{add some motivation}
% We choose a network topology such that there are 2 sets $A$ and $B$ with 4 nodes each such that if the sender of a transaction is in set $A$, then the recipient is in set $B$ and vice versa. Let $\{s,r\}$ be a sender/recipient pair, then there are 3 disjoint paths of lengths $4,5$ and $6$\csr{maybe first try same length} that can be chosen by $s$ to reach $r$ and each $s$ has only these 3 paths to choose from. The timelock of each channel is set to be 1 unit and the balance of every channel is set to be 5000 units in each of its two directions. The value of $t_max$ used in calculating the collateral cost for a transaction is set to be 6 units and $f$ is set to be $0.01$ units. We simulate transactions in sets of 10000 transactions with the transaction numbers $T_{id}$ numbered from 1 to 10000. If the value of $T_{id}\%3$ is 0 or 1, we set the transaction value to be a random integer amount between 1 and 5 or else the transaction amount is set to be a random integral amount between 6 and 50. \csr{sounds random?}

To simulate the payment channel network, we first obtained a snapshot of Lightning from \emph{\url{https://ln.fiatjaf.com}} on February 25th, 2023.  The original snapshot had around 30,000 nodes and 80,000 channels. We 
removed channels that no longer exist and nodes without channels, %Afterwards, we had 
leaving us with around 15,000 nodes and around 60,000 channels.
We also observed that the snapshot included fee (base fee and fee rate) and timelock parameters only for around 8,500 channels.
We derived the distributions of the provided fee and timelock values and then sampled values for the remaining channels independently from the three distributions. 
%Note that we selected from the three distribution independently.

 The sender and recipient of every payment are sampled randomly from a subset of the network $\omega$ of size 10. 
 Once the sender/recipient pair of a payment has been selected, the payment amount is selected. The main use case for payment channel networks is for payments of smaller values. Small payments are most suitable because blockchain fees for conducting payments on-chain do not depend on the payment value and thus executing smaller payments on-chain are more expensive as compared to larger payments~\footnote{\tiny{https://www.coindesk.com/layer2/paymentsweek/2022/04/26/the-lightning-network-is-bringing-payments-back-to-bitcoin/}}. Keeping this in mind, the payment amount for each payment is sampled uniformly between 5\$  (approximately 16,000 satoshis) and 15\$(approximately 48,000 satoshis). We assume a random delay (chosen uniformly) between 0.1 and 1 minute between consecutive payments.
 
Let us now discuss the selection of the routing game parameters. All parameters discussed here are publicly known to all parties and do not change during the course of a simulation run. Firstly, the value of the \emph{LND} risk factor $r$ is $1.5\cdot 10^{-9}$ by default. The value of $r$ determines how the fee compares with the collateral cost in general and consequently the expected utilitites of senders and intermediaries in payments. We thus determine how the models behave for different values of $r$. The default value used for the probability $P_A$ in LND is $0.6$. 
 The value of the time parameter $t^I_{1/2}$ in the computation of the success probablities is taken to be $30$ minutes, and we set the ratio $\tau = (t_{1/2}^S)/(t^I_{1/2})$ to be $2$.

The following three cases are considered in our evaluations: 1) \textit{Original}: Current Lightning, 2) \textit{ModGuranteed}: The sender incentivizes the intermediary $v_i$ to always lock if they have sufficient funds by setting $x_i=c_i/f_i$ (Case 1 in Section~\ref{sec:modifiedgame}), and 3) \textit{ModIncentivized}: The sender uses beliefs on past failures to set $x_i$ such that the intermediaries $v_i$ are likely to lock (Case 2 in Section~\ref{sec:modifiedgame}).
For each case and parameter setting, we simulate 10 runs of 1000 payments each. 


\subsection{Results}\label{results}



% \begin{table}[]
%     \centering
%     \begin{tabular}{|c|r@{$\pm$}l|r@{$\pm$}l|}

% \hline
% $r$ 
% & \multicolumn{2}{c}{$0.1$} 
% & \multicolumn{2}{c}{$0.3$}\\
% \hline
%          $SR$&0.64&0.05&0.65&0.01  \\
%          \hline
%          $LR$&0.67&0.03&0.69&0.01\\
%          \hline
%          $Fee_{I/C}$&0.031&0.004&0.033&0.008\\
%          \hline
%          $Fee_S$&0.020&0.011&0.023&0.006\\
%          \hline
%     \end{tabular}
%     \caption{Comparison of metrics for $r=0.1$ and $r=0.3$. All four metrics increase when $r$ is increased.}
%     \label{table2}
% \end{table}

We now describe the impact of the various incentives on the success ratio, the lock ratio, as well as the average fees. When the risk factor $r$ was set to $1.5\cdot 10^{-9}$, we observed that the collateral cost was very low in comparison to the fee in nearly 99\% of payments and hence the non-refundable fee was very low. Thus, the case is nearly identical to the original Lightning routing. On the other hand, nearly all payments failed when the risk factor was set to $1.5\cdot 10^{-5}$ as the collateral cost was always higher than the fee. Thus, we only varied the value of $r$ between $1.5\cdot 10^{-6}$, $1.5\cdot 10^{-7}$, and $r=1.5\cdot 10^{-8}$. Here, we focus on the case  $r=1.5\cdot 10^{-7}$.

Table~\ref{table} shows a comparison of the three cases with $P_A = 0.6$ and $\tau=2$. We see that the success ratio of payments increased by around 12.2\% when we used ModGuaranteed instead of Original. The lock ratio also increased similar to the success ratio, namely 15.7\%. We see that the average fee paid by a sender per payment decreased by 6\% and the average fee gained by intermediaries per payment also decreased by 8\%. This decrease was due to the higher number of failed payments for Original, which led to senders choosing paths with higher fees as the bias against paths with recent failures in LND prevents senders from using cheap paths. Even though senders paid partial fees of around $F'_S=2.63$ satoshis  per failed payment when using ModGuaranteed, the difference in the path selection makes up for the extra fees. Thus, at least in the scenarios considered here, having non-refundable fees actually reduced the monetary cost for the sender on average. Intermediaries gained $F'_I=1.37$ satoshis per failed payment, so they benefited from locking as was the goal. The gain was lower than the cost of the sender as the sender typically had to pay multiple intermediaries in a path.

% The average fee received by intermediaries and paid by senders increase by  25.7\% and 10.4\%, respectively.
% The increase is more pronounced for the intermediaries than for the senders. Obviously, the absolute amount of fees paid is the same as the amount received. Intermediaries that only receive a low amount of fees have a high percentage increase and this does not equate a high increase for sender. Thus, the modified incentives seem to improve the situation especially for parties that are disadvantaged by the previous incentives, in that they receive very little fees in Lightning. 
%because they forward different numbers of payments, and intermediaries that are less central and hence route payments less frequently profit more than others. 
%\csg{I don't understand this reason. It may be because the definition of the fees for intermediaries was not completely clear} 
%So, our incentives in particular incentivize players that are unwilling to participate in original Lightning payments. 





For ModIncentivized, Table~\ref{table} displays that the values of $SR$ and $LR$ increased by 9\% and 11.4\%,  respectively, in comparison to Original.
%For ModIncentivized, Table~\ref{table1a} displays that the success ratio increases by 5.9\% in comprison to Original. Similarly, the values of $LR$, $F_I$ and $F_S$ also increase by 7.1\%, 8.7\%, and 6.1\%, respectively. 
Although the difference to Original was less pronounced as for ModGuaranteed, ModIncentivized was closer to ModGuaranteed than to Original in terms of locking behavior.  
The results indicate that the sender can choose values of $x_i$ that are lower than $c_i/f_i$ and still expect the payment to succeed. The decrease compared to ModGuaranteed can be attributed to senders not knowing the exact payment history of intermediaries and choosing $x_i$ that were too low to convince the intermediaries to lock. The values of $F_I$ and $F_S$ for ModIncentivized were similar to ModGuaranteed. 
The average income per failed payment for an intermediary was 0.37 satoshis, which is considerably less than for ModGuaranteed, with the sender also paying only about 0.73 satoshis for every failed payment. The difference is to be expected due to the senders choosing lower non-refundable fees. 

 

% When $P_A$ is increased from $0.6$ to $0.8$, the beliefs on success probabilities of channels are scaled up by 33\% as by Eq.~\ref{eq:p}. It is then expected that the values $SR$ and $LR$ increase because a higher \csg{it seems more logical to say "higher" twice}\csp{updated} value of $P_A$ corresponds to a higher success probability $p^i_S$.   Table~\ref{table1b} confirms this expectation. We can also see that for ModIncentivized, $F_I$ and $F_S$ decrease when $P_A$ increases because the value of the non-refundable fee paid by the sender decreases (as intermediaries are more optimistic on payment success, senders can pay lower partial fees). However, this relation does not hold for Original and ModGuaranteed, because there are no non-refundable fees in Original and the non-refundable fees do not depend on $P_A$ in ModGuaranteed.
% Indeed, as confirmed by Table~\ref{table1}, there is no significant difference between $P_A=0.6$ and $P_A=0.8$ for Original and ModGuaranteed. ModGuaranteed and ModIncentivized both achieve notably higher success ratios than Original for both values of $P_A$. 
 


% We further observed in Table~\ref{table2} that when we change the value of $r$ from $0.1$ to $0.3$ (for $t^I_{1/2}=50$, $t_{1/2}^S=200$ and $Pr_A=0.6$) in \textbf{Case 3}, the values of $SR$, $LR$, $Fee_{I\C}$ and $Fee_S$ increases as a higher $r$ implies a higher non-refundable fee for an intermediary on choosing $L$ and thus the average fee paid by the sender and the average fee received increases.  Since, the intermediary is better incentivized to choose $L$, the values of $SR$ and $LR$ also increase. 

% \begin{figure}
% \vspace{-2em}
%     \centering
%     \subfloat[$SR$ and $LR$]{\includegraphics[scale=0.20]{figures/sr.png}\label{SRLR}}
%     \subfloat[$Fee_{I/C}$ and $Fee_S$]{\includegraphics[scale=0.20]{figures/fee-2.png}\label{fee} }
%     \vspace{-1em}
%     \caption{Comparison of metrics for varying values of the ratio $\tau$ for ModIncentivized. Figure~\protect\ref{SRLR} shows how $SR$ and $LR$ change with $\tau$ and Figure~\protect\ref{fee} shows how $F_I$ and $F_S$ change with $\tau$}
%     \label{figure6}
% \end{figure}

% Let us now observe how the metrics are affected by different values of the ratio $\tau$ of the time parameters for the senders and the intermediaries when ModIncentivized is used. 
% Note that the value of $\tau$ does not affect ModGuaranteed as the sender always chooses the partial fee as $c_i/f_i$ and intermediaries are always incentivized to lock. 
% When the value of $\tau$ is increased, i.e., when $t_{1/2}^S$ is higher, the value of $p'^i_S$ increases at a slower rate by Eq.~\ref{eq:p}. Consequently, the $x_i$ that the sender proposes is  more likely to be sufficient for $v_i$ to lock. As a result, the non-refundable fee increases and in turn leads to an increase in the value of all four metrics. Figure~\ref{figure6} depicts this increase by varying $\tau$ between 2 and 8. 
% Indeed, this increase almost closes the gap between ModGuaranteed and ModIncentivized. \csg{where do we see this?}

\begin{figure}
    \centering
    \includegraphics[scale=0.25]{figures/probing.png}
    \vspace{-1em}
    \caption{The cost for the probing attack for different values of the balance to be inferred in ModGuaranteed. The plot shows both the actual probing cost (in blue) for a particular balance and the sliding average (in orange) for every window of 500,000 satoshis.}
    \label{figprob}
    \vspace{-2em}
\end{figure}

Finally, we evaluated the cost for a malicious sender to conduct a probing attack. 
The attacker followed the ModGuaranteed case for choosing the fee because once the first failure occurs, it had to set the partial fee to $c_i/f_i$ as otherwise, a rational intermediary did not lock. 
Here, we considered a path $(v_0,v_1,v_2)$ where $v_0$ is the malicious sender that tried inferring the forwarding balance that $v_1$ had in its channel with $v_2$. The capacity of the channel $(v_1,v_2)$ was chosen to be 4.6 million satoshis, which is the average channel capacity in Lightning\footnote{\tiny{https://1ml.com/statistics}}. The value of the timelock (or $T_1$) between $v_1$ and $v_2$ was 144 blocks, the default value in Lightning. The balance between $v_1$ and $v_2$ was varied between 0 and the channel capacity and we evaluated the \emph{probing cost} in terms of partial fees needed. The probing attack is essentially a binary search to find the balance, with each search iteration being a fake payment. The probing costs is defined as the total non-refundable fees paid for the fake payments.  

Figure~\ref{figprob} shows the cost for the sender to conduct a probing attack. The total fee paid shows an increasing trend with the balance and the cost is roughly 1500 satoshis for every million satoshis in the balance amount probed. While there is an increasing trend, there is no monotonous increase in cost with the balance. The reason is that one of the factors determining the cost is the number of iterations in which $v_1$ had sufficient balance to lock and was paid a non-refundable fee is not strictly increasing. In addition, the probing cost also depends on the total number of iterations needed for the attack, which is again not strictly increasing. 


In summary, we have thus shown that our new incentive model increases the success of payments, as expected. There is no increase in monetary costs for the sender. The new incentive model can also help to deter probing attacks. 















==> ICPADS-Satwik/Introduction.tex <==
\section{Introduction}

%Major cryptocurrencies like Bitcoin~\cite{nakamoto2012bitcoin} and Ethereum~\cite{Buterin2013} are permissionless in nature resulting in limited transaction throughput as compared to centralized systems like Visa.  Thus,  permissionless cryptocurrencies need to find solutions to their scalability issues to cater to a growing user base.  
%Motivation 
Payment channel networks have emerged as a predominant solution to the scalability issues~\cite{gervais2016security} of Bitcoin~\cite{nakamoto2012bitcoin} and Ethereum~\cite{Buterin2013}.
They achieve better scalability, latency, and energy efficiency by offloading transactions between two users from the blockchain to an off-chain layer. 
Lightning, a payment channel network on top of Bitcoin with a liquidity of more than 100 million US dollar, has recently been adopted by some companies for real-world and real-time payments~\footnote{\tiny{https://bitcoinmagazine.com/culture/how-lightning-network-events-bring-adoption}}.

 % Despite the Bitcoin price dropping in May 2022, Lightning investments reached an all-time high on February 23 this year~\footnote{https://www.benzinga.com/news/22/05/27467113/lightning-network-capacity-touches-all-time-high-despite-recent-lackluster-bitcoin-price-action}. 

%Background 
 

%Two blockchain users open a channel by depositing funds 
%on the blockchain in a shared account. 
%Both users can then conduct transactions locally as often as needed as long as they do not exceed the funds locked in the channel.  Each transaction updates the local state by changing the balances on both sides.  The channel can be closed unilaterally by one of the parties or through mutual agreement between both parties as per the latest state.  Hence,  direct interaction between parties is only needed for opening or closing a channel as well as for resolving disputes regarding channel balances.  



%problem 
Multi-hop payments in Lightning are conducted using a two-phase protocol. During this two-phase protocol, senders and intermediaries are required to lock coins that cannot be used for other payments. Thus, intermediaries may be unable to start payments on their own or participate in other payments, meaning there is a collateral cost associated with locking. The cost depends on the amount of coins locked and the duration for which the coins are locked.
The sender pays intermediaries a small fee for locking coins. However, as the fee is only paid upon success, it is not guaranteed that the fee is a sufficient compensation. 

Consequently, it  can  be  a  desirable choice for rational intermediaries to not participate in payments if payments fail frequently. Failed payments can be a result of attacks. For instance, during \textit{probing attacks}~\cite{probing2022Nisslmueller,probing2019herrera,probing2020gijs,probing2020tikhomorov,Biryukov2021probing}, malicious parties attempt to infer the distribution of coins in one or more channels by repeatedly initiating payments via the channel(s) and then intentionally failing them after getting  feedback whether on they are possible. 

%our solution

%Such malicious  behavior  can  be  discouraged  by  our  modification since  the  senders  of  fake  payments  now  need  to  pay  part  of the fees as well. We theoretically derive the additional cost required to conduct a probing attack for a malicious sender and analyze typical costs through simulations.
Our contribution in this paper is two-fold: First, we game-theoretically analyze the existing incentives for intermediaries in Lightning to participate in payments. We assume rational intermediaries who only lock if their expected utility, that is the fee gained minus the collateral cost, exceeds 0. They estimate their expected fee based on previous observations of payment success probability. We determine a \emph{Bayesian Nash Equilibrium}, where all parties act consistently with their beliefs to maximize their expected gain. %Note that locking might not be the optimal strategy in the Bayesian Nash Equilibrium, depending on the beliefs.
Second, we modify the incentives such that partial non-refundable fees (smaller than the routing fee) are paid to intermediaries who lock, even if a payment fails. The complete routing fee is paid for payments that succeed.  We analyze the modified incentives game-theoretically and determine the respective Bayesian Nash Equilibrium. 
A payment sender has two options for choosing the partial fee. It can choose the partial fees such that intermediaries always have a positive utility, even for failed payments, guaranteeing that intermediaries always lock if they have sufficient funds. 
Alternatively, it can also aim to maximize its utility by paying a lower partial fee such that intermediaries are expected to have a positive utility but may not, due to inaccurate beliefs. In this case, intermediaries may refuse to lock. Our analysis is applicable to any source routing payment mechanism that uses a two-phase protocol based on locking and unlocking like Lightning.
 

We evaluate the concrete effect of our modified incentives on rational players in a simulation study. We find that these modified incentives increase the success ratio of payments by up to 12\%. The average routing fees for senders also decreases by up to 6\% as in the original Lightning model, recent payment failures of cheap paths force senders to choose more expensive paths. Our modified incentives model avoids this to some degree as intermediaries of cheaper paths have a higher incentive to participate in payments. Moreover, we find that our modified incentives result in a notable cost for probing attacks. If the balance in one direction of a channel is $n$ million satoshis, we find that the attacker requires approximately $1500n$ satoshis in fees to infer the balance. 
With over 4000 Bitcoin~\footnote{\tiny{https://1ml.com/statistics}} locked in Lightning, a widespread attack when applied to the complete network amounts to tens of thousands  of US dollars in cost.   

%   In this paper, we game-theoretically analyze the incentives for intermediaries in Lightning with the fees and the collateral cost comprising the utilities. In the game theoretic model, senders and intermediaries use knowledge of past payment failures to compute success probability of the current payment and calculate their expected utilities. A rational intermediary locks payment only if its expected utility is greater than zero. We also propose and analyze a modification allowing intermediaries to be payed a part of the routing fee (non-refundable) for locking the payment and fulfilling its  obligation  to  route  the  payment. In doing so, an intermediary is  compensated in case the payment fails at a subsequent intermediary and hence its expected utility is increased. Based on our analysis, we propose guidelines as to how much partial fees is ideal to incentivize intermediaries as well as limit the sender's losses. 

% We test these guidelines through simulation and analyze how paying partial fees to intermediaries affects the rate of success of payments, an intermediary's decision on whether to route the payment or not, the additional monetary cost borne by the sender (since the sender is now paying partial fees when the payment fails) as well as the additional income to the intermediary.
 
%  Such malicious  behavior  can  be  discouraged  by  our  modification since  the  senders  of  fake  payments  now  need  to  pay  part  of the fees as well. We theoretically derive the additional cost required to conduct a probing attack for a malicious sender and analyze typical costs through simulations.

% \textit{griefing attacks}~\cite{griefing2020zohar,mizrahi2021congestion,perez2020lockdown,rohrer2019discharged,congestion2020Lu}, where malicious parties take advantage of the locking mechanism to spam the network with fake payments to  keep  the  funds  of  one  or  many  channels  locked and consequentially unavailable to use for genuine payments, and \textit{probing attacks}~\cite{probing2022Nisslmueller,probing2019herrera,probing2020gijs,probing2020tikhomorov,Biryukov2021probing}, where malicious parties attempt to  infer the balance distribution of channels in the network. Such malicious  behavior  can  be  discouraged  by  our  modification since  the  senders  of  fake  payments  now  need  to  pay  part  of the fees as well.




==> ICPADS-Satwik/Limitations.tex <==
\section{Limitations}
In our current simulation setup, we assume certain parameters like the \emph{LND} risk factor $r$ and the apriori success probability $P_A$ are publicly known and identical for all parties. While there are default values in the Lightning implementation, parties may change them to better reflect their individually perceived risk. Parties with a low amount of funds may consider the same collateral cost less acceptable than those that have a lot of liquidity. 

 While we are in line with Lightning's failure treatment in our predictions of success probabilities, their choice is not based on in-depth studies of various methods, which should be done in future work.  Alternatively, other game theoretic methods like \emph{correlated equilibrium}~\footnote{\tiny{https://en.wikipedia.org/wiki/Correlated_equilibrium}} and \emph{auction theory}~\footnote{\tiny{https://en.wikipedia.org/wiki/Auction_theory}} can also be used to analyze Lightning's fee model. While modifying strategies using the success probabilities (as we do) can be considered as a correlated equilibrium, an external party (like a watchtower) can help parties modify their strategies more efficiently to result in a correlated equilibrium at the cost of privacy. Intermediaries can also choose the non-refundable fee in an auction-like manner. However, communication overhead may become an important factor when considering auctions.

Most notably, we did not consider how to realize the non-refundable fees cryptographically, i.e., integrate them into HTLCs. We leave this to future work as it is beyond the scope of our paper. 



% \csp{Changed} The key idea of the new protocol is to use one HTLC payment for each partial fee. The main difference is that a separate secret and hash is generated for every intermediary's non-refundable fee. The sender includes the hashes for the partials fees in the message about the main payment. They are onion-encrypted such that the non-refundable fee hash $R_i$ for node $v_i$ can be decrypted by its successor $v_{i+1}$. $v_{i+1}$ is then supposed to reveal the hash to $v_i$ so that they can claim their fee after the coins for the main payment have been locked in the channel $(v_i, v_{i+1})$. In this manner, $v_i$ obtains their partial fee for locking.  

% The challenge lies in enforcing that $v_{i+1}$ reveals the hash if and only if $v_i$ chooses the move $L$. We can incentivize $v_{i+1}$ to reveal the hash by delaying the locking of their own partial fee payment until after the hash is provided. Concretely, each partial fee payment to a node $v_{i+1}$ needs to be locked in each of the first $i+1$ channels, so if $v_i$ refuses to lock the partial fee, $v_{i+1}$ cannot receive a partial fee. Hence a rational $v_{i+1}$ always provides the partial fee if they can lock. If they cannot lock, they are not eligible for a partial fee, so they are not directly incentivized here. This case can be handled by having $v_i$ cancel the channel if $v_{i+1}$ does not cooperate. In contrast, the proposed protocol does not prevent $v_{i+1}$ from sharing the hash with its predecessor without locking. This is a serious limitations as it allows nodes to collude and share the partial fees without actually locking. Zero-knowledge proofs that show that locking happened are an avenue for future work.  







==> ICPADS-Satwik/ModifiedRoutingGame.tex <==
\section{Routing with Modified Incentives}
\label{sec:modifiedgame}
The current incentive model does not compensate intermediaries for their participation if the payment fails.  If the collateral cost is too high, a rational intermediary may reason to ignore the payment if it believes that the payment is likely to fail.  We propose an alternative model where an intermediary is paid a portion of the fee if it locks the payment amount on its outgoing channel regardless of whether the payment is successful, thus incentivizing intermediaries to lock payments. We analyze the new fee model from a game-theoretical perspective. 

\subsection{Modified Incentive Model}
Let us consider a payment with path $(v_0,v_1,\ldots,v_n)$ of length $n$. In the original model, the intermediary $v_i$ is paid a fee of $f_i$ if the payment succeeds.  We suggest a modification in which the intermediary receives a fee of $x_i\cdot f_i$ if it locks coins regardless of whether the payment succeeds, where $0\leq x_i\leq 1$ is called the \emph{non-refundable fraction}. If the payment succeeds, the remainder of the fee is paid. Here the value of $x_i$ is chosen by the sender $v_0$ and is communicated to the intermediaries during the locking phase together with the payment value $\alpha_i$. Note that the value of $x_i$ can be different for different intermediaries as they may have different collateral costs. The changes to the incentive model only affect the behavior of parties during the locking phase as they are still incentivized to receive funds during the unlocking phase. Thus, the game tree looks identical to Figure~\ref{figorig} but with different utilities. 

Concretely, the intermediary $v_i$ is guaranteed a utility of $x_i\cdot f_i -c_i$ if it chooses to lock during the locking phase when the payment fails and $f_i-c_i$ if the payment succeeds. So, if $v_i$ decides not to lock the payment, then an intermediary $v_j$ that precedes $v_i$ in the payment path has a utility of $x_j\cdot f_j -c_j$ and the sender has a utility of $-c_0-\sum_{j=1}^{i-1}x_j\cdot f_j$. 
Figure~\ref{figmod} displays the game from the perspective of the intermediary $v_i$, analogously to Figure~\ref{figorig}. 

% The incentives here are modified so that an intermediary $v_i$ receives a partial fee of $x_i\cdot f_i$ if it chooses $L$ and the payment fails, i.e., if nature chooses fail. 

Senders have two options for choosing the value $x_i$. First, they can choose it such that the payment is guaranteed to succeed if balances are sufficient.
However, the fees charged in this case may be higher than necessary. 
Second, the sender can choose the non-refundable fraction $x_i$ such that intermediaries should lock according to the sender's beliefs, leading to lower non-refundable fees than the first option. However, if the sender's beliefs are incorrect, that may lead to failed payments due to the intermediary not having a positive utility according to their beliefs. 
We now discuss the utilities for both cases. For this, let $u^{non}_i$ be the utility function of $v_i$. 

\subsubsection{Case 1: Guaranteed to lock}
Here, the strategy is to set $x_i$ such that $x_i\cdot f_i >c_i$ (note that since $c_i<f_i$, we will find a suitable $x_i$ in $[0,1]$ for all $i$. 
If the value of $x_i\cdot f_i$ is greater than $c_i$ --- or in other words, the utility for $v_i$ on locking $u^{non}_i(L) = x_i\cdot f_i  - c_i>0$ --- then $v_i$ is incentivized to lock regardless of whether the payment succeeds or fails after forwarding.  Thus, $v_i$ will choose $L$ if $x_i\cdot f_i>c_i$.  

\subsubsection{Case 2: Expected to lock} 
Here, the strategy for the sender is to set $x_i$ high enough so that the payment is expected to succeed based on the sender's beliefs, given that there are sufficient funds available. If $x_i\cdot f_i\leq c_i$, then $v_i$ has to consider its belief on $p^i_S$ and $p^i_F$ to calculate its expected utilities on payment success and failure, respectively. As before, $u^{non}_i(NL) = 0$. Its expected utility on choosing $L$ is $u^{non}_i(L) = p^i_S\cdot (f_i - c_i) + p^i_F \cdot (x_i\cdot f_i - c_i)$.
% \begin{align}
% \label{eq:uilM}
% u^{non}_i(L) = p^i_S\cdot (f_i - c_i) + p^i_F \cdot (x_i\cdot f_i - c_i)
% \end{align}
The intermediary $v_i$ hence locks the amount if $u^{non}_i(L)>0$. 
           
% Since the collateral costs $c_i$ decrease with $i$,  the intermediary $v_i$ can be sure that all subsequent nodes in the path will behave honestly and the payment succeeds unless the payment fails due to balance constraints. Thus, $v_i$ can confidently behave honestly if $u_i(H)>0$.


% Thus, an equilibrium is reached here where all the intermediaries choose $L$ when the sender always sets $x_i = \Bar{x}_i$ such that $\Bar{x}_i\cdot f_i$ is higher than $c_i$ for intermediary $v_i$. If the sender chooses a lower value of $x_i$, then the probability that $v_i$ chooses $NL$ increases and the expected utility of the sender decreases as it might lose the large utility of $U$. If the intermediary chooses $NL$, it is choosing a dominated strategy. Hence, no party benefits by changing its strategy.


While the sender can afford to set $x_i$ as 
in Case 1 because of the high success utility $U$, it can also choose a lower value of $x_i$ (lower than $c_i/f_i$) if it is not willing to lose a large part of its fee. As long as $u^{non}_i(L)>0$ for all intermediaries $v_i$ and channel funds are sufficient, the payment is still expected to succeed.  Based on past observations, the sender has a belief $\Tilde{p}^i_S$ i.e., an estimate of $v_i$'s $p^i_S$. Note that the estimate $\Tilde{p}^i_S$ does not change if $v_i$ refuses to lock as it only is concerned with the success probability after $v_i$ chooses to lock. 

By replacing $p^i_S$ by $\Tilde{p}^i_S$ in our computation $u_i^{non}(L)$, we estimate the value $\Tilde{x}_i$ of $x_i$ for which $u^{non}_i(L)$ equals $0$, i.e., if $x_i = \Tilde{x}_i$, $v_0$'s estimate of $v_i$'s expected utility is zero. Choosing $x_i > \Tilde{x}_i$ is hence necessary for $u^{non}_i(L)>0$, at least according to $v_0$'s belief. However, $v_0$ only is aware of the payments of which it has been the sender. If $v_0$'s belief is not in line with the actual success rate observed by $v_i$, $v_i$ might still not lock and the beliefs need to be updated. 
So, $v_0$ sets the value of $x_i = d_i + \Tilde{x}_i$ or $x_i=1$ if $d_i + \Tilde{x}_i>1$, where $d_i$ is a buffer that increases when $v_i$ does not lock and decreases otherwise, thus the term $d_i$ adapts to new information. We explore ways to choose and adapt $d_i$ in Section~\ref{sec:evaluation}. 



%Similar to Section~\ref{ext}, we can assume that the sender always strongly prefers a successful payment and sets $x_i$ accordingly. Calculations for the sender's utility are provided in Appendix~\ref{appsenutil}. 

% We can now determine the expected utilities $u^{non}_0(NL)$ and $u^{non}_0(L)$ for the sender $v_0$. The utility for $v_0$ on choosing $NL$ is $u^{non}_0(NL)=0$. 
% Note that if $v_i$ does not lock and all $v_j$ for $j=1,2,\ldots,i-1$ do lock, $v_0$ has to pay $\sum_{j=1}^{i-1} x_j f_j$ in fees. The probability for this scenario is $P^i_F \left(\prod_{j=1}^{i-1} P^j_S\right)$, i.e., the product of the probabilities for the first $i-1$ \csg{$i-1$ ?}\csp{updated} intermediaries locking and intermediary $v_i$ not locking. We can compute the expected utility in case of failure by summing over all possible $v_i$ that can cause the failure. If the payment is successful, the utility of $v_0$ is the same as for original Lightning. Consequently, 
% \begin{align}
% \begin{split}
%     u^{non}_0(L) &= P_S\cdot \left(U-c_0-\left(\sum_{i=1}^{n-1}f_i\right)-\alpha \right) \\
%     &- \sum_{i=1}^{n-1}P^{i}_F\cdot \left(\prod_{j=1}^{i-1}P^j_S\cdot \left(c_0 +\sum_{k=1}^{i-1} x_k\cdot f_k\right)\right)
% \end{split}
% \end{align}

% \csg{In the second term, I would also put parentheses around the second factor. And shouldn't $x_i \cdot f_1$ all the way at the end not be $x_k \cdot f_k$?}\csp{updated}

In this case, if all intermediaries choose $L$ or $NL$ when their beliefs indicate that $u^{non}_i(L)$ is greater than or less than $0$, respectively,  we have a Bayesian Nash Equilibrium. Similar to the original Lightning protocol, the mixed strategy equilibrium of the routing game is the same as the pure strategy equilibrium.

% The utility for $v_0$ on choosing $NL$ is $u^{non}_0(NL)=0$. 
% Note that if $v_i$ does not lock and all $v_j$ for $j=1,2,\ldots,i-1$ do lock, $v_0$ has to pay $\sum_{j=1}^{i-1} x_j f_j$ in fees. The probability for this scenario is $P^i_F \left(\prod_{j=1}^{i-1} P^j_S\right)$, i.e., the product of the probabilities for the first $i-1$ intermediaries locking and intermediary $v_i$ not locking. We can compute the expected utility in case of failure by summing over all possible $v_i$ that can cause the failure. If the payment is successful, the utility of $v_0$ is the same as for original Lightning. Consequently, 
% \begin{align}
% \begin{split}
%     u^{non}_0(L) &= P_S\cdot \left(U-c_0-\left(\sum_{i=1}^{n-1}f_i\right)-\alpha \right) \\
%     &- \sum_{i=1}^{n-1}P^{i}_F\cdot \prod_{j=1}^{i-1}P^j_S\cdot \left(c_0 +\sum_{k=1}^{i-1} x_k\cdot f_k\right)
% \end{split}
% \end{align}
%allowing mixed strategies results in pure strategies unless the utility of locking is 0, in which case all strategies was the same utility. 
 

% In contrast to the Lightning protocol, our modification allows the source to provide extra incentives to an intermediary for whom choosing $L$ seems not to be a dominant strategy. We demonstrate how the modified incentives improve the rate of success of payments and the average extra income provided to the intermediaries in Section~\ref{results}. We further show that the average increased cost for the sender remains much lower than the average transaction fee in the Bitcoin network.

% So far we have discussed how non-refundable fees change the game theory of payment channel networks and encourage parties to lock funds. In addition, the HTLC protocol applied in Lightning needs to be modified to cryptographically realize the protocol. The modifications do not require advanced smart contracts and can hence be integrated into Lightning. The modified HTLC protocol we propose in Appendix~\ref{appcrypto} guarantees intermediaries their non-refundable fee paid by the source if they lock coins in the subsequent channel.

\subsection{Disincentivizing Probing Attacks}
 In a probing attack (detailed description in Section~\ref{secprobing}), a source uses multiple fake payments to learn the available balance in a channel. 
In the original protocol, the sender does not incur any monetary losses while attempting fake payments. However, with the modified incentives the sender has to pay partial fees whenever the intermediary chooses $L$. Given that a probing attack typically consists of many payments, the intermediary is bound to have a low value for its estimate $p^i_S$ of the probability of a successful payment after locking. Most likely, excluding the first few payments, the source has to choose $x_i\cdot f_i>c_i$ for a rational intermediary to lock. The modified incentives also disincentivize griefing attacks with malicious intermediaries refusing to lock payments as now the non-refundable fees are an opportunity cost for these attackers.


% \subsection{Effect against attacks}

% We now show how the modified incentive model mitigates the impact of griefing and probing attacks. \csr{you have to cite the papers about the attacks}

% \subsubsection{Griefing attacks}
% The main idea of a griefing attack as discussed in Section~\ref{attacks} is for an attacker to freeze channel balances in the network and create a Denial of Service scenario either to stop activity in the network or to divert payments from competing channels to itself. To conduct such an attack, the attacker must initiate fake payments that it does not intend to fulfil. In the original incentives model, the cost for a griefing attack was the cost involved in opening channels with nodes whose channel balances, the attacker wanted to freeze\csr{not necessarily, you can open channels with other nodes and then construct a path via a channel that it wants to freeze}. In the modified incentives model, the attackers have an additional cost in terms of the partial fees paid to intermediaries on locking the payment amount and hence, fake payments come at a cost. The attacker could indeed choose to keep the value of $x$ low. In this case, the intermediaries chooses not to forward the payment as it is not incentivized to do so and hence the attack fails. Thus, to mount a successful attack, the intermediary needs to maintain the value of $x$ so that intermediary nodes feel incentivized to forward payments and the attacker is successful. Thus, the modified incentives model increases the cost of conducting griefing attacks.\csr{well, that is obvious; it's more a motivation, might want to have it earlier}

% \subsubsection{Probing attacks}
% In a probing attack, the attacker sends probes (fake payments) of various payment amounts to infer the balance distribution of its chosen target channels. Similar to griefing attacks, the attacker again has to pay partial fees to intermediaries while doing fake payments, maintaining the value of $x$ and each probe has some additional cost associated with it. Thus, the modified incentives model increases the cost of conducting probing attacks. \csr{again: obvious; some deeper insights, e.g., how do you compute the cost, assuming that values are known? }

==> ICPADS-Satwik/Related.tex <==
\section{Related Work}
%We first discuss previous research on the game-theoretic analysis of payment channel networks followed by a summary of alternate fee models. Then, we present other approaches to mitigate the effects of or prevent probing attacks. 
% Finally, we discuss approaches that enable reduced collateral cost through alternative cryptographic constructions. 

Several recent works~\cite{avarikioti2019creationgames,Avarikioti_2020ride,rain2021gametheoretic} provide a game-theoretic analysis on different aspects of  payment channel networks. Payment channel networks are treated as creation games in~\cite{avarikioti2019creationgames} and~\cite{Avarikioti_2020ride} where the authors discuss the trade-offs between the creation costs of channels and the fees collected by routing payments. They further analyze various network topologies and determine the fee policies that constitute a Nash equilibrium for each network topology. 
A related work not based on game theory shows how a party can adapt its fee rates to maximize traffic under the assumption that other parties keep their fees as they are~\cite{Ersoy_2020_profit}. However, their results are not applicable when all parties act rational.  

The notion of using extensive form games to analyze payment channel networks to find Bayesian equilibriums was explored in~\cite{rain2021gametheoretic,ZhangGT, mazumdar2022strategic}. The authors in~\cite{rain2021gametheoretic} analyze the security properties of channel closing and multi-hop HTLC payments. They particularly focus on the strategies for both channel parties during the channel closing game and formally characterizing the Wormhole attack~\cite{Malavolta2019AnonymousML} in the routing game. Zhang et.al.~\cite{ZhangGT} analyzes payment channel networks game theoretically in terms of resilience to rational deviations and immunity to Byzantine behaviors. Additionally, the paper also analyzes opening, closing and normal operation of payment channels. However, both works do not consider the negative utilities induced by collateral costs in the routing game. Moreover, they ignore the aspect that intermediaries in payment channel networks do not know the complete payment path and treat the routing game as a game with complete information. \csp{New}The authors in~\cite{mazumdar2022strategic} analyze the intermediaries’ decisions based on the presence of corrupt nodes as a game between two intermediaries. Our model considers all parties involved in the payment including the sender. While we do not model corrupt nodes, we accommodate cases where payments fail due to insufficient balances (which makes identifying corrupt behavior harder).

% Cross-chain swaps, which can also use HTLCs, and Nash equilibriums of existing cross-chain swaps are explored in~\cite{crosschainGT}. However, they do not consider multi-hop payments. 


A parallel work to ours proposes to defend against probing attacks using differential privacy~\cite{van2022hiding}. In contrast to our approach, the defense requires an additional circular noise payment to obfuscate the payment value and hence the inference of the balance. The additional payment requires that more nodes lock collateral, which --- as by our analysis --- some might refuse. 
To date, the work is only the defense against probing attacks.

%There are a number of related attacks. Tochner et al.\ present a game-theoretic analysis of denial-of-service attacks where intermediaries aim to block payments by not locking~\cite{tochner2019hijacking}. They find that an attacker can set its fees low to attract more parties to route via it and hence severely degrade the success probability of payments. 

Like probing attacks, \emph{griefing attacks}~\cite{griefing2020zohar,mizrahi2021congestion,perez2020lockdown,rohrer2019discharged,congestion2020Lu} also exploit the locking mechanism. Instead of privacy, they target the availability of the system by forcing intermediaries to lock funds for as long as possible, preventing the use of these funds in actual payments.
Mazumdar et.al~\cite{counter2020mazumdar,mazumdar2022strategic} propose an alternative HTLC construction that penalizes the node responsible for the griefing attack (intermediary or recipient). Honest victims of the attack are compensated based on its total timelock and the cumulative compensation of all honest victims is paid by the attacker. The alternative HTLC construction involves the creation of two contracts: a penalty contract is set up from the receivers' side whereas the normal payment contract is set up from the sender's side. Thus, it is different to our construction in that our contracts are all set up from the sender side. Furthermore, in our protocol, the sender ---being the attacker in a probing attack --- pays fees for locking whereas in their protocol, the attacker is an intermediary or the receiver and hence the extra fees are not paid by the sender.   

Similar to~\cite{counter2020mazumdar}, the concept of reverse-bond was proposed in~\cite{upfrontreversebond}. The reverse-bond proposal is a mechanism in which a party that accepts a HTLC pays a hold (or rent) fee for the duration that it holds the HTLC. However, there is no proposal on how this can be realized formally and how the hold duration can be tracked accurately. The concept of up-front fees was discussed in~~\cite{nonrefundable,upfront}. However, these proposals were dismissed stating that the solution doesn't avoid the attack and senders might have to pay large upfront fees for small payments.
Several mitigation strategies for griefing like enforcing faster HTLC resolution, loop avoidance, shorter paths and non-refundable fees were suggested in~\cite{mizrahi2021congestion} without any follow-up on how they can be achieved. 

% Finally, attempts have also been made to use alternate cryptographic constructions for reducing the collateral costs in multi-hop payments and hence improving incentives for both senders and intermediaries in payment paths. Sprites~\cite{miller2017sprites} reduces the collateral by having a constant total timelock for all channels in a payment path, so the total collateral of the payment is linear with respect to the path length. Atomic Multi-Channel Updates~\cite{Egger2019amcu} and Payment Trees~\cite{jourenko2021trees} further improves on this to provide constant collateral payments. 



==> ICPADS-Satwik/RoutingGame.tex <==
\section{Analysis of Lightning's Routing}
\label{rout}

Let us now evaluate Lightning's routing algorithm from a game-theoretical perspective. We derive the conditions that incentivize rational intermediaries to lock payments. 

\subsection{Assumptions}
We assume that all parties act rationally and try to maximize their gains from every payment they participate in.  So, we exclude parties that become unresponsive due to being offline. In addition, we consider malicious behavior when we analyze the probing attack by a malicious sender. 
All payments are assumed to be multi-hop and source routed using \emph{LND} protocol. The utilities for intermediaries and senders depend on the routing fee and the collateral cost incurred by locking. 
% In Section~\ref{sec:pcn}, we introduced the notion of the collateral cost for an intermediary in a multi-hop payment, and routing fee as a compensation for this cost. 
Since a party sets its base fee and fee rate, it can select their values to be high enough so that fees are always greater than the collateral cost.
%(intermediaries refuse payments that have a collateral cost higher than the maximum possible collateral cost) \csg{do we know what this maximum is?}\csp{I explain this in terms of $T_{max}$ in the next paragraph}. 

Let $(v_0,v_1,\ldots,v_n)$ be a payment in which $v_0$ is sending an amount $\alpha$ to $v_n$, $c_i$ denote $v_i$'s worst-case collateral cost and $T_i=\sum_{j=i}^{n-1}t_i$ denote the cumulative timelock from $v_i$ to $v_n$. In the rest of the paper, we use the terms collateral cost and worst-case collateral cost interchangeably.
The sender initially sends payment value $\alpha_0 = \alpha + \sum_{j=1}^{n-1} f_j$ and each step reduces the payment value by $f_i$, the fees of intermediary $i$. Thus, the amount that $v_{i}$ pays to $v_{i+1}$ in a successful payment is $\alpha_i = \alpha + \sum_{j=i+1}^{n-1} f_j$. In particular, $\alpha_{n-1}=\alpha$.  
The collateral cost $c_i=T_i\cdot \alpha_i\cdot r$ is obtained as described in Section~\ref{seccost}, where $r$ is the \emph{LND} risk factor. 
% know that $c_i$ is $\mathcal{O}(T_i\cdot \alpha_i)$ and the proportional fee portion already takes the payment amount $\alpha_i$ into account. The maximum possible collateral cost is reached when the timelock $T_i$ is equal to $T_{max}$, the maximum possible timelock (we assume $T_{max}$ is public knowledge). Keeping this in mind, we set the collateral cost $c_i$ to be $({T_i}/{T_{max})f_i}$,
% which can easily be calculated if $T_i$, $\alpha_i$ and the fee parameters $b_i$ and $p_i$ are known.


Since the sender knows the payment path, it can calculate the value of $c_i$ for all intermediaries. The sender $v_0$ is assumed to benefit with a utility gain $U$ when the payment succeeds that more than compensates its loss of funds (i.e., intermediaries' fees and payment amount) and its collateral cost, which is $\alpha\cdot T_0\cdot r$.
%and we have $U>>\alpha \cdot T_0$ to discourage senders from backing out of payments. \csg{is this a conclusion or a requirement?}\csp{updated}
Additionally, when a payment fails, the sender knows the exact failure link. This knowledge is useful for the sender to find paths that have a high probability of succeeding and used by Lightning's LND routing algorithm to reduce failures\footnote{\tiny{https://github.com/lightningnetwork/lnd}}.


\begin{figure*}
%\vspace{-3.5em}
\centering


%\begin{istgame}
%\setistgrowdirection'{west}
%   \xtdistance{20mm}{40mm}
%   \istroot(0){$v_0$}
%     \istb{I}[above left]{(0,0,0,0)}
%     \istb{H}[above right]
%     \endist
%   \istroot(1)(0-2)<10>{$v_1$}
%     \istb{I}[al]{(-c_0,0,0,0)}
%     \istb{H}[ar]
%     \endist
%    \istroot(2)(1-2)<10>{$v_2$}
%     \istb{I}[al]{(-c_0,-c_1,0,0)} 
%     \istb{H}[ar]
%     \endist
%     \istroot(3)(2-2)<10>{$v_3$}
%     \istb{I}[al]{(-c_0,-c_1,-c_2,0)} 
%     \istb{H}[ar]
%     \endist
%     \istroot(4)(3-2)<10>{$v_2$}
%     \istb{I}[al]{(-c_0,-c_1,-c_2,U)} 
%     \istb{H}[ar]
%     \endist
%      \istroot(5)(4-2)<10>{$v_1$}
%     \istb{I}[al]{(-c_0,-c_1,f_2-c_2,U)}
%     \istb{H}[ar]
%     \endist
%      \istroot(6)(5-2)<10>{$v_0$}
%     \istb{I}[al]{(-c_0-f_1-f_2,f_1-c_1,f_2-c_2,U)}
%     \istb{H}[ar]{(U-c_0-f_1-f_2,f_1-c_1,f_2-c_2,U)}
%     \endist
%   \end{istgame}
%   \caption{Extensive form Routing Game}
%   \label{figure1}
\begin{tikzpicture}[font=\tiny,scale=0.75]
  % Two node styles: solid and hollow
    \tikzstyle{solid node}=[circle,draw,inner sep=1.2,fill=black];
    \tikzstyle{hollow node}=[circle,draw,inner sep=1.2];
    \tikzstyle{level 1}=[level distance=10mm]
    \tikzstyle{level 2}=[level distance=13mm]
    \tikzstyle{level 3}=[level distance=16mm]
    \tikzstyle{level 4}=[level distance=19mm]
    \tikzstyle{level 5}=[level distance=22mm]
    \tikzstyle{level 6}=[level distance=25mm]
    % \tikzstyle{level 6}={level distance=18mm}
  % The Tree
  \node(0)[hollow node]{}
    child[grow=down]{node[solid node]{}edge from parent node[left]{$NL$}}
    child[grow=right]{node(1)[solid node]{}
      child[grow=down]{node[solid node]{}edge from parent node[left]{$NL$}}
      child[grow=right]{node(2)[solid node]{}
        child[grow=down]{node[solid node]{}edge from parent node[left]{$NL$}}
        child[grow=right]{node(3)[solid node]{}
          child[grow=down]{node[solid node]{}edge from parent node[left]{$DH$}}
          child[grow=right]{node(4)[solid node]{}
            child[grow=down]{node[solid node]{}edge from parent node[left]{$DH$}}
            child[grow=right]{node(5)[solid node]{}
              child[grow=down]{node[solid node]{}edge from parent node[left]{$DH$}}
              child[grow=right]{node(6)[solid node]{}
              edge from parent node[above]{$H$}
              }
            edge from parent node[above]{$H$}
            }
          edge from parent node[above]{$H$}
          }
        edge from parent node[above]{$L$}
        }
      edge from parent node[above]{$L$}
      }
    edge from parent node[above]{$L$}
};


% Movers
%\foreach \x in {0}
%    \node[above]at(\x){$v_0$};
%  \foreach \x in {1,5}
%    \node[above]at(\x){$v_1$};
%  \foreach \x in {2,4}
%    \node[above]at(\x){$v_2$};
%  foreach \x in {3}
%    \node[above]at(\x){$v_3$};
  \node[above]at(0){$v_0$};
  \node[above]at(1){$v_1$};
  \node[above]at(2){$v_2$};
  \node[above]at(3){$v_3$};
  \node[above]at(4){$v_2$};
  \node[above]at(5){$v_1$};
  % payoffs
  \node[below]at(0-1){$(0,0,0,0)$};
  \node[below]at(1-1){$(-c_0,0,0,0)$};
  \node[below]at(2-1){$(-c_0,-c_1,0,0)$};
  \node[below]at(3-1){$(-c_0,-c_1,-c_2,0)$};
  \node[below]at(4-1){\makecell{$(-c_0,-c_1,$\\$-c_2-\alpha_2,U)$}};
  \node[below]at(5-1){\makecell{$(-c_0,-c_1-\alpha_1,$\\$f_2-c_2,U)$}};
  \node[right]at(6){\makecell{$(U-c_0 - f_1-f_2-\alpha,$\\ $f_1-c_1,f_2-c_2,U)$}};
\end{tikzpicture}
\vspace{-0.5em}
\caption{Extensive form game for Lightning's original routing protocol with four nodes. Each edge represents one of four moves: lock $L$, not lock $NL$, provide secret $H$, and withhold secret $DH$. The game begins at $v_0$ and leaf nodes  are tuples of utilities. }
\label{figrout}
\vspace{-2em}
   \end{figure*}









\subsection{Extensive Form Game for Lightning}\label{ext}
%Let us represent a Lightning multi-hop payment as an extensive form game. We first assume that all players use pure strategies and then extend the results to mixed strategies. 
The execution of the payment along a path $(v_0,v_1,\ldots,v_n)$ of length $n$ can be considered as a game with $n+1$ players. This execution consists of a locking phase with the $v_i$ and $v_{i+1}$ for $i=0..n-1$ sequentially locking $\alpha_i$ coins in their channel, followed by an unlocking phase in which all locked coins are released starting from the last channel. 
The sender $v_0$ starts the locking phase by making the first move in the game by locking $\alpha_0$ in the channel $(v_0,v_1)$. Each intermediary $v_i$ makes a move after $v_{i-1}$ has locked $\alpha_{i-1}$ in the channel $(v_{i-1},v_i)$. After the last intermediary $v_{n-1}$ locks $\alpha$ in the channel $(v_{n-1},v_n)$, the locking phase of the payment is completed. An intermediary $v_i$ may choose not to lock during this phase either because it has insufficient funds or it is not sufficiently incentivized. In this case, the payment fails with a worst-case utility loss of $c_j$ for each node $v_j$ preceding $v_i$ in the path. The move of locking a payment is denoted by $L$ and the move of not locking is denoted by $NL$.

After all parties have locked, the recipient $v_{n}$ starts the unlocking phase by providing the payment secret to $v_{n-1}$ and hence unlocking the locked amount in the channel $(v_{n-1},v_n)$. Each intermediary $v_i$ again makes a move when it receives the payment secret from $v_{i+1}$. $v_i$ can now share the secret with $v_{i-1}$ to receive the amount locked in the channel $(v_{i-1},v_i)$ or withhold the secret. The move of revealing the secret is denoted by $H$ and the move of withholding the secret is denoted by $DH$. Once $v_i$ receives the locked amount, its net utility in the game is $f_i-c_i$. If $v_i$ withholds the payment secret, it still has to pay $\alpha_i = \alpha + \sum_{j=i+1}^{n-1} f_j$, so its utility is $-c_i - \alpha_i$. The sender does not need to pay in this case as the intermediary does not claim its coins. 
If all intermediaries choose $H$ and $v_0$ receives the secret from $v_1$, $v_0$'s utility is $U-\sum_{i=1}^{n-1}f_i - \alpha -c_0$. An example of the game for $n=3$ is displayed in Figure~\ref{figrout}.   Clearly, after $v_{n-1}$ has locked the payment on its channel $(v_{n-1},v_n)$, all parties are incentivized to choose $H$ over $DH$. As we assume that all intermediaries are rational, they will always choose $H$ and the game tree can be simplified to the one in Figure~\ref{figreduced}.  



 \begin{figure}
 \centering
\begin{tikzpicture}[font=\tiny,scale=1]
  % Two node styles: solid and hollow
    \tikzstyle{solid node}=[circle,draw,inner sep=1.2,fill=black];
    \tikzstyle{hollow node}=[circle,draw,inner sep=1.2];
    \tikzstyle{level 1}=[level distance=8mm]
    \tikzstyle{level 2}=[level distance=10mm]
    \tikzstyle{level 3}=[level distance=12mm]
  % The Tree
  \node(0)[solid node]{}
    child[grow=down]{node[solid node]{}edge from parent node[left]{$NL$}}
    child[grow=right]{node(1)[solid node]{}
      child[grow=down]{node[solid node]{}edge from parent node[left]{$NL$}}
      child[grow=right]{node(2)[solid node]{}
        child[grow=down]{node[solid node]{}edge from parent node[left]{$NL$}}
        child[grow=right]{node(3)[solid node]{}
edge from parent node[above]{$L$}
              }
            edge from parent node[above]{$L$}
            }
          edge from parent node[above]{$L$}
          };
       
\node[above]at(0){$v_0$};
  \node[above]at(1){$v_1$};
  \node[above]at(2){$v_2$};
\node[below]at(0-1){$(0,0,0,0)$};
  \node[below]at(1-1){$(-c_0,0,0,0)$};
  \node[below]at(2-1){$(-c_0,-c_1,0,0)$};
   \node[right]at(3){\makecell{$(U-c_0 - f_1-f_2-\alpha,$\\ $f_1-c_1,f_2-c_2,\alpha)$}};
   \end{tikzpicture}
   \vspace{-0.5em}
   \caption{Version of Lightning routing game after concluding that $H$ is always a dominant strategy in comparison to $DH$ and hence players always choose $H$.}
   
   \label{figreduced}
   \vspace{-2em}
   \end{figure}
   




  %In other words, we assume that the payment succeeds after the penultimate node locks the payment amount, hence resulting in a positive utility of $f_i$ to every intermediary $v_i$ and the source spends \csg{perhaps "spends", it is not really a loss}\csp{updated} $\sum_{i=1}^{n-1} f_i+ \alpha$ while gaining a utility of $U$ as a reward for the successful payment. \csg{BTW, how is $U$ computed?}\csp{$U$ is a fixed value that is very high}

 

% \begin{figure*}
% \centering
% \begin{tikzpicture}[font=\footnotesize,scale=2]
%   % Two node styles: solid and hollow
%     \tikzstyle{solid node}=[circle,draw,inner sep=1.2,fill=black];
%     \tikzstyle{hollow node}=[circle,draw,inner sep=1.2];
%   % The Tree
%   \node(0)[solid node]{}
%     child[grow=down]{node[solid node]{}edge from parent node[left]{$NL$}}
%     child[grow=right]{node(1)[solid node]{}
%       child[grow=down]{node[solid node]{}edge from parent node[left]{$NL$}}
%       child[grow=right]{node(2)[solid node]{}
%         child[grow=down]{node[solid node]{}edge from parent node[left]{$NL$}}
%         child[grow=right]{node(3)[solid node]{}
% edge from parent node[above]{$L$}
%               }
%             edge from parent node[above]{$L$}
%             }
%           edge from parent node[above]{$L$}
%           };
       
% \node[above]at(0){$v_0$};
%   \node[above]at(1){$v_1$};
%   \node[above]at(2){$v_2$};
% \node[below]at(0-1){$(0,0,0,0)$};
%   \node[below]at(1-1){$(-c_0,0,0,0)$};
%   \node[below]at(2-1){$(-c_0-x_1\cdot f_1,x_1\cdot f_1-c_1,0,0)$};
%   \node[right]at(3){\makecell{$(U-c_0 - f_1-f_2,$\\ $f_1-c_1,$\\ $f_2-c_2,U)$}};
%   \end{tikzpicture}
%   \caption{Simplified extensive form Routing Game with modified incentives. We consider a payment path of length 4. Here if $v_2$ chooses $NL$ after $v_1$ has chosen $L$, then the sender has a net loss of $-c_0-x_1\cdot f_1$ and the intermediary $v_1$ has a net utility of $x_1\cdot f_1 - c_1$.}
   
%   \label{figure4}
%   \end{figure*}
   
% \begin{figure}
% \vspace{-1em}
%     \centering
% \begin{istgame}[font=\tiny,scale=0.75] %\setistgrowdirection'{east} 
% \xtdistance{15mm}{30mm} 
% \istroot(0)<above right>{$N$}
%   \istb{$S$}[al]
%   \istb{$F$}[ar]
%   \endist
% \xtdistance{15mm}{30mm}
% \istroot(1)(0-1)
%   \istb{$L$}[al]{f_i-c_i}
%   \istb{$NL$}[ar]{0}
%   \endist
% \istroot(2)(0-2)
%   \istb{$NL$}[al]{0}
%   \istb{$L$}[ar]{x_i\cdot f_i-c_i}
%   \endist
% \xtInfoset(1)(2){$v_i$}
% \end{istgame}
% \vspace{-1em}
% \caption{Game tree from the perspective of $v_i$ with modified incentives. The only difference here from Figure~\protect\ref{figure3} is that when $v_i$ chooses $L$ when $N$ chooses $F$, $v_i$ gets an additional utility of $x_i \protect\cdot f_i$.}
% \label{figure5}
% \vspace{-2em}
% \end{figure}  

We now game-theoretically analyze the behavior of payment intermediaries. Both pure and mixed strategies are considered, i.e., intermediaries may always choose the same strategy or choose between multiple strategies. We first assume pure strategies and then generalize. 
Lightning uses onion routing~\cite{goldschlag1999onion}, so an intermediary $v_i$ does not know the complete path of a payment. 
Thus, the Lightning routing game is a game with incomplete information. 
Let $S$ and $F$ be the events indicating that a payment is successful or fails, respectively, after $v_i$ locks the payment. From $v_i$'s perspective, the outcome between $S$ and $F$ is random. However, we assume $v_i$ has a belief on this outcome in the form of probabilities $p^i_S$ and $p^i_F=1-p^i_S$ for success and failure, respectively.
%The probabilities $p^i_S$ and $p^i_F$ 
These probabilities are determined by $v_i$ based on the final outcome of past payments it has forwarded to $v_{i+1}$, including the cases where the payment failed due to insufficient balances.
We show the game tree from the perspective of $v_i$ in Figure~\ref{figorig}. 

Let $u_i(L)$ and $u_i(NL)$ denote the utility that $v_i$ expects when choosing $L$ and $NL$ respectively.  
It is clear that $u_i(NL) = 0$. The utility for $v_i$ in choosing $L$ is $f_i-c_i$ if the payment succeeds and $-c_i$ if the payment fails, so $u_i(L) = p^i_S\cdot (f_i-c_i) - p^i_F\cdot c_i$.
%We can thus calculate the expected utility for $v_i$ when choosing $L$ as 
% \begin{align}
% \label{eq:uiL}
% u_i(L) = p^i_S\cdot (f_i-c_i) - p^i_F\cdot c_i.
% \end{align}
% We can formally define $p^i_S$ as a function $FN$ of its history $HS$\csr{why does $HS$ have subscripts below but not here?} for payments where the node succeeding $v_i$ is $v_{i+1}$, i.e., 
% \begin{align}
% \label{eq:pis}
% p^i_S = FN(HS_{v_{i+1}}^i). 
% \end{align}
Being rational parties, the intermediaries choose $L$ only if the utility for locking is higher than for not locking. Thus, an intermediary $v_i$ forwards the payment only if $u_i(L)>0$. For a successful payment i.e., for locking to be the strategy chosen by all players, we require $u_i(L)>0$ for $i=0,1,\ldots,n$. When each player chooses $L$ only if its beliefs suggest that its utility on choosing $L$ is positive, we have a Bayesian Nash equilibrium. 

Let us now assume that $v_i$ adopts a mixed strategy and assigns probabilities $p_L$ and $p_{NL}$ to the strategies $L$ and $NL$, respectively, with $p_L+p_{NL}=1$. The expected utility of $v_i$ here is $u^m_i=p_L\cdot u_i(L) + p_{NL}\cdot u_i(NL) = p_L\cdot u_i(L)$. We observe that $u^m_i$ is increasing  if $u_i(L)$ is greater than zero and decreasing if it is less than zero. Hence, as long as $u_i(L) \neq 0$, $v_i$ does always adapt a pure strategy, even if mixed strategies are possible. If $u_i(L)=0$, all mixed strategies have the same expected utility, namely 0. 

Since the sender uses the same path-finding protocol as used in \emph{LND}, the exact utility of the sender is not a factor in its decisions. So, we skip the sender's utility computation in this paper.

% From Section~\ref{secroute}, we know that the sender chooses a path with low collateral cost and high success probability. The sender gets an additional utility of $U>>c_0\cdot \alpha_0$ . We let $P^i_S$ and $P^i_F=1-P^i_S$ be the sender's belief on whether $v_i$ locks the amount with $v_{i+1}$ based on its past payment history with $v_i$.The payment is successful if all intermediaries choose $L$. $v_0$'s belief of the probability for a successful payment is  $P_S = \prod_{i=1}^{n-1}P^i_S$ and the probability of failure is $P_F=1-P_S$. 
% By the utilities discussed above, $v_0$'s expected utility on choosing $L$ is hence
% \begin{align}
% \label{eq:u0L}
% u_0(L) = P_S\cdot \left(U-c_0-\alpha -\sum_{i=1}^{n-1}f_i \right) - P_F\cdot c_0. 
% \end{align}

% Detailed calculation of the sender's utilities is provided in Appendix~\ref{appsenutil}. 








% We can similarly calculate the utilities for the sender $v_0$ on moves $L$ and $NL$. Note that $v_0$ is unaware of payments made by other senders that also go through $v_i$ and $v_{i+1}$. Furthermore, whenever choosing $NL$ for a payment, $v_i$ and not $v_0$ is aware of the reason for doing so, i.e., insufficient balance or negative utility. \csg{are you implying here that the sender does not know this?}\csp{Essentially yes. I explicitly mentioned it now} Thus, the sender's beliefs on the value of $p^i_S$ considered by $v_i$ is not reliable. We let $P^i_S$ and $P^i_F=1-P^i_S$ be the sender's belief on whether $v_i$ locks the amount with $v_{i+1}$ based on past payments sent by the sender as it knows points of payment failures. \csg{I don't understand this sentence. How does the sender know $P_S^i$ and $P_F^i$?}\csp{Basically when a payment fails, the sender knows that the payment fails at $v_i$ say, then it can update $P_F^i$ accordingly}

% (Note that the sender . Similar to Equation~\ref{eq:pis}, we get \csr{now HS has two subscripts, before it had one? and you never explained what they mean, please be consistent and define your notation}
% \begin{align}
% \label{eq:PiS}
% P^i_S = FN(HS_{v_i,v_{i+1}}^0). 
% \end{align}
% Note that $v_0$ can only consider payments between $v_i$ and $v_{i+1}$ that it is aware of. Due to the use of onion routing, $v_0$ only knows its predecessor and successor on the path if it is not the source of the payment. Thus, the only payments between $v_i$ and $v_{i+1}$ with $i > 0$ that $v_0$ can consider in its history are payments it is the source of. In contrast, $v_i$ is aware of all payments it made to $v_{i+1}$.  $v_0$ is not aware of the reason. Thus, $P^i_S \neq p^i_S$.  

% The payment is successful if all intermediaries choose $L$. $v_0$'s belief of the probability for a successful payment is  $P_S = \prod_{i=1}^{n-1}P^i_S$ and the probability of failure is $P_F=1-P_S$. 
% By the utilities discussed above, $v_0$'s expected utility on choosing $L$ is hence
% \begin{align}
% \label{eq:u0L}
% u_0(L) = P_S\cdot \left(U-c_0-\alpha -\sum_{i=1}^{n-1}f_i \right) - P_F\cdot c_0. 
% \end{align}






\begin{figure}
    \centering
\subfloat[Original incentives]{
\begin{istgame}[font=\tiny,scale=0.5] %\setistgrowdirection'{east} \
\xtdistance{15mm}{30mm} 
\istroot(0)<above right>{$N$}
  \istb{$S$}[al]
  \istb{$F$}[ar]
  \endist
\xtdistance{15mm}{30mm}
\istroot(1)(0-1)
  \istb{$L$}[al]{f_i-c_i}
  \istb{$NL$}[ar]{0}
  \endist
\istroot(2)(0-2)
  \istb{$NL$}[al]{0}
  \istb{$L$}[ar]{-c_i}
  \endist
\xtInfoset(1)(2){$v_i$}
\end{istgame}

\label{figorig}
}
\subfloat[Modified incentives]{
\centering
\begin{istgame}[font=\tiny,scale=0.5] %\setistgrowdirection'{east} 
\xtdistance{15mm}{30mm} 
\istroot(0)<above right>{$N$}
  \istb{$S$}[al]
  \istb{$F$}[ar]V
  \endist
\xtdistance{15mm}{30mm}
\istroot(1)(0-1)
  \istb{$L$}[al]{f_i-c_i}
  \istb{$NL$}[ar]{0}
  \endist
\istroot(2)(0-2)
  \istb{$NL$}[al]{0}
  \istb{$L$}[ar]{x_i\cdot f_i-c_i}
  \endist
\xtInfoset(1)(2){$v_i$}
\end{istgame}
\label{figmod}
}
\vspace{-0.5em}
\caption{Game tree from the perspective of $v_i$, only showing $v_i$'s utility. $v_i$ cannot be sure whether the payment succeeds ($S$) or fails ($F$) after $v_i$ chooses $L$ ($N$ denotes a random choice here). The differences in the utilities of the original and modified incentives are also illustrated}. 
\vspace{-3em}
\label{figint}


\end{figure} 
% For a successful payment to correspond to a Bayesian Nash Equilibrium,  
% Whether locking is indeed a Bayesian Nash Equilibrium depends on the historical data in the concrete payment channel network, so we evaluate it in a simulation in Section~\ref{sec:evaluation}. 

==> ICPADS-Satwik/appresults.tex <==
\section{Additional Results}\label{app}

\begin{table*}
\centering
\subfloat[$r=1.5\cdot 10^{-6}$\label{table1a}]{
\centering
	\begin{tabular}{c r@{$\pm$}l r@{$\pm$}l r@{$\pm$}l r@{$\pm$}l r@{$\pm$}l r@{$\pm$}l}
		\toprule
		\textit{Cases} 
		& \multicolumn{2}{c}{$SR$} 
		& \multicolumn{2}{c}{$LR$}
		& \multicolumn{2}{c}{$F_I$}
		& \multicolumn{2}{c}{$F_S$}
		& \multicolumn{2}{c}{$F'_I$}
		& \multicolumn{2}{c}{$F'_S$}\\
		\midrule
		\textbf{\textit{Original}} & 0.25&0.06 & 0.28&0.06 & 7.08&0.33&16.69&1.88&0&0&0&0\\
        \textbf{\textit{ModGuaranteed}} & 0.39&0.08 & 0.44&0.07 &5.83&0.51 &14.91&0.97&10.29&2.6&12.38&3.44\\
		\textbf{\textit{ModIncentivized}} & 0.37&0.08 & 0.41&0.07 & 5.81&0.51&15.44&1.35&4.69&1.53&5.73&2.01\\
		\bottomrule
	\end{tabular}
 
    }
 \hfill
 \subfloat[$r=1.5\cdot 10^{-8}$\label{table1b}]{
 \centering
	\begin{tabular}{c r@{$\pm$}l r@{$\pm$}l r@{$\pm$}l r@{$\pm$}l r@{$\pm$}l r@{$\pm$}l}
		\toprule
		\textit{Cases} 
		& \multicolumn{2}{c}{$SR$} 
		& \multicolumn{2}{c}{$LR$}
		& \multicolumn{2}{c}{$F_I$}
		& \multicolumn{2}{c}{$F_S$}
		& \multicolumn{2}{c}{$F'_I$}
		& \multicolumn{2}{c}{$F'_S$}\\
		\midrule
		\textbf{\textit{Original}} & 0.83&0.04 & 0.90&0.02 & 2.30&0.23&9.77&2.03&0&0&0&0\\
        \textbf{\textit{ModGuaranteed}} & 0.88&0.03 & 0.95&0.02 &2.11&0.21 &9.71&2.13&0.17&0.03&0.32&0.05\\
		\textbf{\textit{ModIncentivized}} & 0.85&0.03 & 0.93&0.02 & 2.07&0.2&9.76&2.17&0.03&0.01&0.05&0.02\\
		\bottomrule
	\end{tabular}
    }
 \caption{Comparison of metrics in the three cases Original, ModGuaranteed, and ModIncentivized for different values of the risk factor $r$.}
\end{table*}
In this section, we evaluate how changing the value of $r$ affects the metrics defined in Section~\ref{metrics}. Table~\ref{table1a} displays the results when $r$ is $1.5\cdot 10^{-6}$, so a factor 10 lower than the value used in Section~\ref{sec:evaluation}. The values of $SR$ and $LR$ are lower as the values seen in Table~\ref{table} and the values of the fee metrics are higher.  We notice the same trend as in Section~\ref{results} with a high success ratio and lock ratio achieved when using ModGuaranteed. We also see that the difference between fee models is more pronounced. For a lower value of $r$, the success ratio increased by 56\%. The average amount spent by a sender on fees also decreased by 10.5\% as compared to 6\% in Section~\ref{results}. The income earned as non-refundable fee per failed payment by an intermediary increased by a factor of 3. Senders spend on average more than five times as much on fees. 

On the flip side, we see in Table~\ref{table1b} that when $r=1.5\cdot 10^{-8}$, then the values of $SR$ and $LR$ increase as compared to when $r=1.5\cdot 10^{-7}$ as intermediaries are more likely to lock payments. Again, we observe the same trend as in Section~\ref{results} with a high success ratio and lock ratio achieved when using ModGuaranteed. However, for a low value of $r$, the success ratio achieved by Original was very close to ModGuaranteed and ModIncentivized. ModGuaranteed only showed an improvement of 6\% over Original. The values of the fee metrics decreased compared to $r=1.5\cdot 10^{-7}$, especially for the non-refundable fees. 

==> ICPADS-Satwik/figures/htlc.tex <==
\begin{tikzpicture}[scale=0.7,font=\tiny]
\draw[fill=blue, opacity=0.1,text opacity=1] (0.2,0) rectangle (1,4) node[pos=.5] {$v_0$};
\draw[fill=blue, opacity=0.1,text opacity=1] (5.2,0) rectangle (6,4) node[pos=.5] {$v_1$};
\draw[fill=blue, opacity=0.1,text opacity=1] (10.2,0) rectangle (11,4) node[pos=.5] {$v_2$};
\draw[fill=blue, opacity=0.1,text opacity=1] (15.2,0) rectangle (16,4) node[pos=.5] {$v_3$};
\node at (-1,3) {main};
\draw (1,3) -- node [midway,above]{$HTLC2\left(\alpha_0, h(r), h(r_0)\right)$}(5.2,3);
\draw (6,3) -- node [midway,above]{$HTLC2\left(\alpha_1, h(r), h(r_1)\right)$}(10.2,3);
\draw (11,3) -- node [midway,above]{$HTLC2\left(\alpha_2, h(r), h(r_2)\right)$}(15.2,3);
\node at (-1,2) {fee $v_1$};
\draw (1,2) -- node [midway,above]{$HTLC\left(x_1\cdot fee(v_1), h(r_1)\right)$}(5.2,2);
\node at (-1,1) {fee $v_2$};
\draw (1,1) -- node [midway,above]{$HTLC\left(x_2\cdot fee(v_2), h(r_2)\right)$}(5.2,1);
\draw (6,1) -- node [midway,above]{$HTLC\left(x_2\cdot fee(v_2), h(r_2)\right)$}(10.2,1);
\end{tikzpicture}

==> appresults.tex <==
\section{Additional Results}\label{app}

\begin{table*}
\centering
\subfloat[$r=1.5\cdot 10^{-6}$\label{table1a}]{
\centering
	\begin{tabular}{c r@{$\pm$}l r@{$\pm$}l r@{$\pm$}l r@{$\pm$}l r@{$\pm$}l r@{$\pm$}l}
		\toprule
		\textit{Cases} 
		& \multicolumn{2}{c}{$SR$} 
		& \multicolumn{2}{c}{$LR$}
		& \multicolumn{2}{c}{$F_I$}
		& \multicolumn{2}{c}{$F_S$}
		& \multicolumn{2}{c}{$F'_I$}
		& \multicolumn{2}{c}{$F'_S$}\\
		\midrule
		\textbf{\textit{Original}} & 0.25&0.06 & 0.28&0.06 & 7.08&0.33&16.69&1.88&0&0&0&0\\
        \textbf{\textit{ModGuaranteed}} & 0.39&0.08 & 0.44&0.07 &5.83&0.51 &14.91&0.97&10.29&2.6&12.38&3.44\\
		\textbf{\textit{ModIncentivized}} & 0.37&0.08 & 0.41&0.07 & 5.81&0.51&15.44&1.35&4.69&1.53&5.73&2.01\\
		\bottomrule
	\end{tabular}
 
    }
 \hfill
 \subfloat[$r=1.5\cdot 10^{-8}$\label{table1b}]{
 \centering
	\begin{tabular}{c r@{$\pm$}l r@{$\pm$}l r@{$\pm$}l r@{$\pm$}l r@{$\pm$}l r@{$\pm$}l}
		\toprule
		\textit{Cases} 
		& \multicolumn{2}{c}{$SR$} 
		& \multicolumn{2}{c}{$LR$}
		& \multicolumn{2}{c}{$F_I$}
		& \multicolumn{2}{c}{$F_S$}
		& \multicolumn{2}{c}{$F'_I$}
		& \multicolumn{2}{c}{$F'_S$}\\
		\midrule
		\textbf{\textit{Original}} & 0.83&0.04 & 0.90&0.02 & 2.30&0.23&9.77&2.03&0&0&0&0\\
        \textbf{\textit{ModGuaranteed}} & 0.88&0.03 & 0.95&0.02 &2.11&0.21 &9.71&2.13&0.17&0.03&0.32&0.05\\
		\textbf{\textit{ModIncentivized}} & 0.85&0.03 & 0.93&0.02 & 2.07&0.2&9.76&2.17&0.03&0.01&0.05&0.02\\
		\bottomrule
	\end{tabular}
    }
 \caption{Comparison of metrics in the three cases Original, ModGuaranteed, and ModIncentivized for different values of the risk factor $r$.}
\end{table*}
In this section, we evaluate how changing the value of $r$ affects the metrics defined in Section~\ref{metrics}. Table~\ref{table1a} displays the results when $r$ is $1.5\cdot 10^{-6}$, so a factor 10 lower than the value used in Section~\ref{sec:evaluation}. The values of $SR$ and $LR$ are lower as the values seen in Table~\ref{table} and the values of the fee metrics are higher.  We notice the same trend as in Section~\ref{results} with a high success ratio and lock ratio achieved when using ModGuaranteed. We also see that the difference between fee models is more pronounced. For a lower value of $r$, the success ratio increased by 56\%. The average amount spent by a sender on fees also decreased by 10.5\% as compared to 6\% in Section~\ref{results}. The income earned as non-refundable fee per failed payment by an intermediary increased by a factor of 3. Senders spend on average more than five times as much on fees. 

On the flip side, we see in Table~\ref{table1b} that when $r=1.5\cdot 10^{-8}$, then the values of $SR$ and $LR$ increase as compared to when $r=1.5\cdot 10^{-7}$ as intermediaries are more likely to lock payments. Again, we observe the same trend as in Section~\ref{results} with a high success ratio and lock ratio achieved when using ModGuaranteed. However, for a low value of $r$, the success ratio achieved by Original was very close to ModGuaranteed and ModIncentivized. ModGuaranteed only showed an improvement of 6\% over Original. The values of the fee metrics decreased compared to $r=1.5\cdot 10^{-7}$, especially for the non-refundable fees. 

==> figures/htlc.tex <==
\begin{tikzpicture}[scale=0.7,font=\tiny]
\draw[fill=blue, opacity=0.1,text opacity=1] (0.2,0) rectangle (1,4) node[pos=.5] {$v_0$};
\draw[fill=blue, opacity=0.1,text opacity=1] (5.2,0) rectangle (6,4) node[pos=.5] {$v_1$};
\draw[fill=blue, opacity=0.1,text opacity=1] (10.2,0) rectangle (11,4) node[pos=.5] {$v_2$};
\draw[fill=blue, opacity=0.1,text opacity=1] (15.2,0) rectangle (16,4) node[pos=.5] {$v_3$};
\node at (-1,3) {main};
\draw (1,3) -- node [midway,above]{$HTLC2\left(\alpha_0, h(r), h(r_0)\right)$}(5.2,3);
\draw (6,3) -- node [midway,above]{$HTLC2\left(\alpha_1, h(r), h(r_1)\right)$}(10.2,3);
\draw (11,3) -- node [midway,above]{$HTLC2\left(\alpha_2, h(r), h(r_2)\right)$}(15.2,3);
\node at (-1,2) {fee $v_1$};
\draw (1,2) -- node [midway,above]{$HTLC\left(x_1\cdot fee(v_1), h(r_1)\right)$}(5.2,2);
\node at (-1,1) {fee $v_2$};
\draw (1,1) -- node [midway,above]{$HTLC\left(x_2\cdot fee(v_2), h(r_2)\right)$}(5.2,1);
\draw (6,1) -- node [midway,above]{$HTLC\left(x_2\cdot fee(v_2), h(r_2)\right)$}(10.2,1);
\end{tikzpicture}
